STAMP: Scalable Task And Model-agnostic Collaborative Perception

Perception is crucial for autonomous driving, but single-agent perception is often constrained by sensors' physical limitations, leading to degraded performance under severe occlusion, adverse weather conditions, and when detecting distant objects. Multi-agent collaborative perception offers a solution, yet challenges arise when integrating heterogeneous agents with varying model architectures. To address these challenges, we propose STAMP, a scalable task- and model-agnostic, collaborative perception pipeline for heterogeneous agents. STAMP utilizes lightweight adapter-reverter pairs to transform Bird's Eye View (BEV) features between agent-specific and shared protocol domains, enabling efficient feature sharing and fusion. This approach minimizes computational overhead, enhances scalability, and preserves model security. Experiments on simulated and real-world datasets demonstrate STAMP's comparable or superior accuracy to state-of-the-art models with significantly reduced computational costs. As a first-of-its-kind task- and model-agnostic framework, STAMP aims to advance research in scalable and secure mobility systems towards Level 5 autonomy. Our project page is at https://xiangbogaobarry.github.io/STAMP and the code is available at https://github.com/taco-group/STAMP.

==> sec/2_related_works_bk.tex <==
\section{Related Works}

\subsection{Multi-agent Collaborative Perception}
Multi-agent collaborative perception has been developed to overcome occlusions and perception range limitations inherent in single-agent perception systems~\cite{hu2022investigating}. 
%
There are three main information-sharing schemas in multi-agent collaborative perception systems: early fusion, intermediate fusion, and late fusion. 
%
Early fusion~\cite{gao2018object, chen2019cooper, arnold2020cooperative} involves sharing raw sensor data (e.g., LiDAR, camera) directly between agents. While this approach maximizes information transfer, it is often considered impractical for real-world applications due to high bandwidth requirements.
%
Late fusion~\cite{rauch2012car2x, caltagirone2019lidar, melotti2020multimodal, fu2020depth, zeng2020dsdnet, shi2022vips, glaser2023we, xu2023model}, on the other hand, involves sharing only final prediction results, such as object detection bounding boxes or occupancy predictions. This method minimizes communication bandwidth overhead but often leads to suboptimal accuracy. Additionally, late fusion is task-dependent, meaning models with different tasks are not collaborative. 
%
Intermediate fusion methods~\cite{chen2017multi, mehr2019disconet, marvasti2020cooperative, wang2020v2vnet, liu2020when2com, liu2020who2com, guo2021coff, bai2022pillargrid, cui2022coopernaut, lei2022latency, xu2022cobevt, xu2022v2x, qiao2023adaptive, li2023learning, wang2023core, wang2023vimi, yu2023vehicle} share mid-level information, such as Bird's Eye View (BEV) features, between agents. This approach strikes a balance between communication bandwidth and information loss, making it the most promising fusion strategy. However, intermediate fusion faces significant challenges in addressing domain gap issues for heterogeneous agents.

\subsection{Collaborative Perception for Heterogeneous Agents}

\noindent In a heterogeneous collaborative perception scenario, we assume there are \( N \) hetero agents ready for collaboration. An agent \( i \) usually consists of an encoder \( E_j \), a collaborative fusion layer \( U_i \), and a decoder \( D_i \), each receiving the input data \( I_i \) where \( k \in \{1, 2, \ldots, i\} \). For annotation simplicity, we assume all models receive input from the same number of agents, without losing generality for different agent numbers. 

Upon receiving the input data \( I_i \), the encoder \( E_i \) maps it to the BEV feature \( F_i \). Each agent's BEV feature \( F_i \) is then broadcast to other agents within the collaborative distance \( d \), which is the maximum distance for two agents to collaborate. The collaborative fusion layer \( U_i \) gathers and fuses the BEV features from all collaborating agents, resulting in the fused BEV feature \( F' \). Finally, the decoder \( D_i \) decodes the fused BEV feature \( F' \) to produce the final model output \( O_i \). This procedure is formulated as follows:

% \begin{equation}
% O_k = D_k(F'_k),\ \text{where}\ F_k = E_k(I_k),\ F'_k = U_k(F_{1:K}),\ \text{for } k \in \{1, 2, \ldots, K\}.
% \end{equation}

% \begin{equation}
%     \begin{aligned}
%     F_k &\leftarrow E_k(I_k), \\
%     F'_k &\leftarrow U_k(F_{1:K), \\
%     O_k &\leftarrow D_k(F'_k), \quad \text{for } k \in \{1, 2, \ldots, K\}.
%     \end{aligned}
% \end{equation}


\begin{align}
&\text{Encoding:} \quad F_i = E_i(I_i), \quad \forall i \in \{1, 2, \ldots, N\}, \label{eq:encoding}\\
&\text{Fusion:} \quad F'_i = U_i(\{F_k ~|~\mathcal{N}(i, k) \leq d\}), \quad \forall i \in \{1, 2, \ldots, N\}, \label{eq:fusion}\\
&\text{Decoding:} \quad O_i = D_i(F'_i), \quad \forall i \in \{1, 2, \ldots, N\}. \label{eq:decoding}
\end{align}

where $\mathcal{N}(i, k)$ refers to the Euclidean distance between the agent $i$ and agent $k$.

\noindent\textbf{Model and Agent Heterogeneity:} In collaborative perception scenario, two agents are called heterogeneous (hetero) agents if they are equipped with hetero models, where two models are heterogeneous in three levels: 1) hetero modalities~\cite{xiang2023hm,lu2024extensible}; 2) hetero model architectures or parameters, and~\cite{xu2023model} 3) hetero downstream tasks, with each refers the heterogeneity in \Eqrefs{eq:encoding}{eq:fusion}{eq:decoding}, respectively. 

% \XG{Do we need this line?}
% Note that for homogeneous perception, we assume $E_k$, $U_k$, and $D_k$ are the same for all agents, where \Eqref{eq:hetero_cav} can be simplified to $O = D \circ U\left(E(I_1), E(I_2), \ldots, E(I_K)\right)$.

For 1) hetero modalities, two models are expected to take input data $I_k$ of different modalities, such as RGB image or lidar point clouds, which requires to use different encoders $E_k$ to process them to BEV features $F_k$ of different representations which are non-collaborative. \cite{xiang2023hm} propose hetero-modal vision transformer to fuse heterogeneous BEV features, but requires end-to-end model training which is not practical for existing hetero agents. \cite{lu2024extensible} propose back-ward alignment training strategy, which requires training a base network first, then, fix the decoder of the base network and train encoders only to create hetero models. This technics enables collaboration between existing hetero agents, but still has high computational cost especially for models with large encoders. \cite{xu2023bridging} proposes Multi-agent Perception Domain Adaption (MPDA), conducting pair-wised adaptation to align the feature map between two hetero agents. Their method effectively make hetero agents collaborative but requires polynomial complexity respect to the number of hetero models, therefore not scalable. For 2) hetero model architecture or parameters, both encoder $E_k$ and fusion model $U_k$ for each model is not required to be the same, which results in multiple fused BEV feature $F'_k$ in different domains. In this case, both $F_k$ and $F'_k$ are not required to be in the same domain, so existing hetero intermediate fusion methods~\cite{xiang2023hm, lu2024extensible} are not applicable. However since $O_k$ for all models are in the same domain, late fusion methods~\cite{xu2023bridging} are still applicable. Finally, hetero downstream tasks refers to the case where all encoder $E_k$, fusion model $U_k$, and decoder $D_k$ different among each model. This is the hardest case where even $O_k$ for all model are not required to be in the same domain. To our knowledge, our proposed pipeline is the first work that address all three cases.  \XG{yiming has a paper to do task agnostic CAV\cite{li2023multi}, which we need to explain}



% In this section, we choose two late fusion methods, vanillan late fusion, and calibrator~\cite{xu2023model}, along with two intermediate fusion methods End-to-end training, and HEAL~\cite{lu2024extensible} for comparing with our heterogeneous collaborative perception pipeline existing pipelines on the 3D object detection task. In collaborative 3D object detection, using late fusion instead of intermediate fusion is a simple way to alleviate the domain gap. ~\cite{xu2023model} claims that their is still domain gap in late fusion due to the difference of training data and training details among each heterogeneous model, therefore use a calibrator to fill in this domain gap in the decision space. For intermediate fusion, one way to avoid the domain gap is to use end-to-end training. That is, training all heterogeneous models together and let them collaborate during the training stage to fill in the domain gap. However, this training strategy is not only costly in training and usually takes much larger epochs to converge, but also not extensible after finishing training. ~\cite{lu2024extensible} propose backward alignment technics, train a base network first, then, fix the decoder of the base network and train encoders only to create heterogeneous models. That is, all models share the same decoder. This technics enables new hetero agents to join in, but not scalable \XG{}. 



==> sec/3_methodology_bk_bk.tex <==

\section{Methodology}

\subsection{Overview}

Our proposed framework, STAMP, enables collaboration among existing heterogeneous agents without sharing model details or downstream task information. 
%
We replace the compression (\Eqref{eq:compression}) and decompression (\Eqref{eq:decompression}) with adaptation and reversion steps. Specifically, for each agent $i$, we introduce a local adapter $\upphi_i$ and a local reverter $\uppsi_i$. The adaptation process is defined as follows:
\begin{equation}
\text{Adaptation:} \quad F_{iP} = \upphi_i(F_i), \quad \forall i \in \{1, 2, \ldots, N\} \label{eq:adaptation}
\end{equation}
Here, the adapter $\upphi_i$ maps the local BEV feature $F_i$ to a unified BEV feature representation, which we term the protocol feature, denoted as $F_P$. The resulting adapted feature is denoted as $F_{iP}$.

Following adaptation, the features from all heterogeneous agents $i$ are broadcast to other agents $j$ within the collaborative distance $d$. Each receiving agent $j\  (j\neq i$) then uses its local reverter $\uppsi_j$ to map the received features back to its own local feature representation. The resulting reverted features are denoted as $F_{ij}$. This reversion process is formulated as:
\begin{equation}
\text{Reversion:} \quad F_{ij} =
\begin{cases}
\uppsi_j(F_{iP}), & \text{if } i \neq j \\
F_i, & \text{if } i = j
\end{cases}
\quad \forall i, j \in \{1, 2, \ldots, N\}\label{eq:reversion}
\end{equation}
Note that $F_i$ is already in the local feature presentation so stay intact. This adaptation and reversion process seamlessly integrates into the standard heterogeneous collaborative perception pipeline, forming the core of our STAMP framework.


\begin{figure*}[t]
\includegraphics[width=\textwidth]{Figures/pipeline.pdf}
\vspace{-7mm}
\caption{Initially, agents are non-collaborative (I), resulting in degraded performance. CFA (II) enables collaboration among heterogeneous agents through a two-step process: training a protocol network and training local adapters and reverters. The \textcolor{red}{protocol network} facilitates communication between \textcolor{blue}{Agent 1}, \textcolor{green}{Agent 2}, and \textcolor{yellow}{Agent 3}, each with heterogeneous models and features. Gradient-colored feature maps represent features adapted or reverted between domains. After CFA implementation, agents become collaborative (III), leading to improved performance.}
\label{figure:pipeline}
\vspace{-3mm}
\end{figure*}


\subsection{Collaborative Feature Alignment}
\label{sec:collab_adapt}

To train a unified BEV feature representation and a local adapter-reverter pairs, we propose \textbf{Collaborative Feature Alignment (CFA)}. As illustrated in \Figref{figure:pipeline} (I), before CFA, heterogeneous agents perform multiple tasks individually without the ability to collaborate, resulting in suboptimal performance. After CFA (III), these agents can effectively collaborate, leading to a significant performance boost.

% \subsubsection{Training Protocol Network}
\paragraph{Training protocol network.}The first step is to learn a unified BEV embedding space by training a protocol network. This process follows the standard collaborative perception model training, as described in \Cref{eq:encoding,eq:compression,eq:decompression,eq:fusion,eq:decoding}. We denote the protocol encoder, fusion model, and decoder as $E_P$, $U_P$, and $D_P$, respectively. The compressor and decompressor are set to be identity. The input data, BEV feature, fused BEV feature, and final output of the protocol model are represented by $I_P$, $F_P$, $F'_P$, and $O_P$, respectively. It's important to note that the protocol model is not restricted to any specific architecture or downstream task, thus being a task and model-agnostic framework.


\paragraph{Training local adapters and reverters.}We introduce a notation $\mathcal{X}=\{\mathbf{x}^1, \mathbf{x}^2, \hdots, \mathbf{x}^K\}$ to denote a set of \textbf{world states}, where $K$ is the total number of world states. A modality transformation function $\mathcal{T}:\mathcal{X} \to I$ transforms a world state to sensor data of a given modality. For instance, in an autonomous driving scenario, $\mathbf{x}$ could represent the world state surrounding the ego vehicle, and $\mathcal{T}$ could be the matrix of six surround-view RGB cameras, resulting in $I$ as the six RGB images captured by these cameras. Given a local model $i$, protocol model $P$, and a set of world states $\mathcal{X}=\{\mathbf{x}^1, \mathbf{x}^2, \hdots, \mathbf{x}^K\}$, we define $I^k_i = \mathcal{T}_i(\mathbf{x}^k)$ as the input for local model $i$ and $I^k_P = \mathcal{T}_P(\mathbf{x}^k)$ as the input for protocol model $P$. Here, $\mathcal{T}_i$ and $\mathcal{T}_P$ denote the sensor modalities of the local model $i$ and protocol model, respectively. 

Consider the local BEV feature $F^k_i=E_i(\mathcal{T}_i(\mathbf{x}^k))$ and protocol BEV feature $F^k_P=E_P(\mathcal{T}_P(\mathbf{x}^k))$. A domain gap exists between these features due to the heterogeneity of sensor modalities $\mathcal{T}_i$ and $\mathcal{T}_P$, and encoders $E_i$ and $E_P$. To bridge this gap, we introduce a local adapter $\upphi_i$ that maps $F^k_i$ to the protocol feature representation:
\begin{equation}
\upphi_i = \argmin_{\upphi_i} \mathfrak{D}_P(F^{1:K}_{iP}, F^{1:K}_P) \quad \text{where} \quad F^k_{iP} = \upphi_i(F^k_i)
\end{equation}
Similiarly, we introduce a reverter $\uppsi_i$ that maps the protocol BEV feature $F^k_P$ to the local feature representation. By including $F^k_{ii} = \uppsi_i(F^k_{iP})$, we provide additional supervision for $\uppsi_i$. We formulate the objective function for $\uppsi_i$ as:
\begin{equation}
\begin{aligned}
& \uppsi_i = \argmin_{\uppsi_i} \left(\mathfrak{D}_i(F^{1:K}_{Pi}, F^{1:K}_i) + \mathfrak{D}_i(F^{1:K}_{ii}, F^{1:K}_i) \right) \\
\text{where} \quad & F^k_{Pi} = \uppsi_i(F^k_P),\ F^k_{ii} = \uppsi_i(F^k_{iP})
\end{aligned}
\end{equation}
The function $\mathfrak{D}_P(\cdot, \cdot)$ and $\mathfrak{D}_i(\cdot, \cdot)$ denote a distance function in the protocol domain and local feature domain of agent $i$, respectively. These two distance metrics are defined considering the feature distance both in the feature space $\mathfrak{D}^f_P(\cdot, \cdot)$, $\mathfrak{D}^f_i(\cdot, \cdot)$ and the decision space $\mathfrak{D}^d_P(\cdot, \cdot)$, $\mathfrak{D}^d_i(\cdot, \cdot)$.


\paragraph{Feature space alignment.}
For a given local model $i$, we first align the feature pairs $(F^k_{iP}, F^k_P)$, $(F^k_{Pi}, F^k_i)$, and $(F^k_{ii}, F^k_i)$ for all $k$ using the $L2$-norm. This direct alignment of feature spaces is formulated as:
\begin{equation}
\begin{aligned}
& L^f_{\upphi_i} = \mathfrak{D}^f_P(F^{1:K}_{iP}, F^{1:K}_P) \overset{\triangle}{=} \frac{1}{K} \sum_{k} \|F^k_{iP}, F^k_P\|_2,\quad \\
& L^f_{\uppsi_i} = \mathfrak{D}^f_i(F^{1:K}_{Pi}, F^{1:K}_i) + \mathfrak{D}^f_i(F^{1:K}_{ii}, F^{1:K}_i) \overset{\triangle}{=} \frac{1}{K} \sum_{k} \left(\|F^k_{Pi}, F^k_i\|_2 + \|F^k_{ii}, F^k_i\|_2\right)
\end{aligned}
\end{equation}
where $L^f_{\upphi_i}$ and $L^f_{\uppsi_i}$ represent the feature space alignment losses for the adapter $\upphi_i$ and reverter $\uppsi_i$, respectively.



\paragraph{Decision space alignment.}In scenarios where $\mathcal{T}_i$ and $\mathcal{T}_P$ differ significantly (e.g., RGB Camera vs. LiDAR), the gap between intermediate feature representations can be substantial. In such cases, achieving exact equality between $F^k_{iP}$ and $F^k_P$ may be neither possible nor necessary. However, since $F^k_i$ and $F^k_{iP}$ originate from the same world state $\mathbf{x}^k$, their downstream task outputs should be aligned. Thus, we define,
% \begin{equation}
% \begin{aligned}
%     & \mathfrak{D}^d_P(F^{1:K}_{iP}, F^{1:K}_P) = \|D_P\circ U_P(F^{1:K}_{iP}), D_P\circ U_P(F^{1:K}_{P})\|_2 \\
%     & \mathfrak{D}^d_i(F^{1:K}_{Pi}, F^{1:K}_i) = \|D_i\circ U_i(F^{1:K}_{Pi}), D_i\circ U_i(F^{1:K}_{i})\|_2 \\
%     & \mathfrak{D}^d_i(F^{1:K}_{ii}, F^{1:K}_i) = \|D_i\circ U_i(F^{1:K}_{ii}), D_i\circ U_i(F^{1:K}_{i})\|_2 \\
% \end{aligned}
% \end{equation}
\begin{equation}
\begin{aligned}
    & \mathfrak{D}^d_P(F^{1:K}_{iP}, F^{1:K}_P) = \|O_{iP}, O_P\|_2,\ \text{where}\ O_{iP} = D_P\circ U_P(F^{1:K}_{iP}), O_{P} = D_P\circ U_P(F^{1:K}_{P}) \\
    & \mathfrak{D}^d_i(F^{1:K}_{Pi}, F^{1:K}_i) = \|O_{Pi}, O_i\|_2,\ \text{where}\ O_{Pi} = D_i\circ U_i(F^{1:K}_{Pi}), O_{i} = D_i\circ U_i(F^{1:K}_i) \\
    & \mathfrak{D}^d_i(F^{1:K}_{ii}, F^{1:K}_i) = \|O_{ii}, O_i\|_2,\ \text{where}\ O_{ii} = D_i\circ U_i(F^{1:K}_{ii}), O_{i} = D_i\circ U_i(F^{1:K}_i) \\
\end{aligned}
\end{equation}

In practical, generating the label $D_P\circ U_P(F^{1:K}_{P})$ and $D_i\circ U_i(F^{1:K}_{i})$ requires extra computational overhead. Consider that $D_P$ and $U_P$ has been trained with learning objective of minimizing $\mathcal{L}_P(O_{P}, ~\text{GT}_P)$ while $D_i$ and $U_i$ has been trained with learning objective of minimizing $\mathcal{L}_i(O_i, ~\text{GT}_i)$ for all $i$, where  $\mathcal{L}_P$ and $\mathcal{L}_i$ represent the loss function been used for training protocol model and local model $i$, respectively, and $\text{GT}_P$ and $\text{GT}_i$ denote the corresponding ground truth labels for the protocol and local model $i$, to 


% Specifically, the outputs of adapted local features $D_P\circ U_P({F^k_{iP}|\forall k})$ and protocol features $D_P\circ U_P({F^k_P~|~\forall k})$ should align with ground truth labels $\text{GT}_P$. The outputs of reverted local features $D_i\circ U_i({F^k_{ii}|\forall k})$, reverted protocol features $D_i\circ U_i({F^k_{Pi}|\forall k})$, and original local features $D_i\circ U_i({F^k_i~|~\forall k})$ should align with ground truth labels $\text{GT}_i$. 



To enforce this alignment in the decision space, we introduce additional loss terms:
\begin{equation}
\begin{aligned}
    & L^d_{\upphi_i} = \mathcal{L}_P(D^P\circ U^P(\{F^k_{iP}~|~\forall k\}),~\text{GT}_P) \\
    & L^d_{\uppsi_i} = \mathcal{L}_i(D^{l_i}\circ U^{l_i}(\{F^k_{Pi}~|~\forall k\}),~\text{GT}_i) + \mathcal{L}_i(D^{l_i}\circ U^{l_i}(\{F^k_{ii}~|~\forall k\}),~\text{GT}_i)
\end{aligned}
\end{equation}
where $\mathcal{L}_P$ and $\mathcal{L}_i$ represent the appropriate task-specific loss functions for the protocol model and local model $i$, respectively. $\text{GT}_P$ and $\text{GT}_i$ denote the corresponding ground truth labels for the protocol and local model tasks. $L^d_{\upphi_i}$ and $L^d_{\uppsi_i}$ represent the decision space alignment losses for the adapter $\upphi_i$ and reverter $\uppsi_i$, respectively.

Finally, to balance the importance of adaptation and reversion, as well as feature and decision space alignment, we introduce scaling factors $\lambda^f_\upphi$, $\lambda^f_\uppsi$, $\lambda^d_\upphi$, and $\lambda^d_\uppsi$. The total loss function for local model $i$ is:
\begin{equation}
L_i = \lambda^f_\upphi L^f_{\upphi_i} + \lambda^f_\uppsi L^f_{\uppsi_i} + \lambda^d_\upphi L^d_{\upphi_i} + \lambda^d_\uppsi L^d_{\uppsi_i}
\end{equation}








% \noindent \textbf{Aligning Decision Space:} Under the case where $\mathcal{T}_i$ and $\mathcal{T}_P$ are hugely different, such as rgb images and lidar point clouds, the resulting large gap between the intermediate feature representations. In this case, it is neither possible nor necessary to find a $\upphi_i$ such that $F^k_{iP}$ to be the same as $F^k_P$. However, because $F^k_i$ and $F^k_{iP}$ share the same physical world information $\mathbf{x}^k$ for all $k$, the downstream task outputs of the adapted local features $D_P\circ U_P(\{F^k_{iP}~|~\forall k\})$ has the same ground truth labels $\text{GT}_P$ as the output of protocol features $D_P\circ U_P(\{F^k_P~|~\forall k\})$. Similarly, the downstream task outputs of the reverted local features $D_i\circ U_i(\{F^k_{ii}~|~\forall k\}))$, reverted protocol feature $D_i\circ U_i(\{F^k_{Pi}~|~\forall k\})$, and the original local features $D_i\circ U_i(\{F^k_i~|~\forall k\}))$ has the the same ground truth labels $\text{GT}_i$. To this end, we propose additional loss to align the features in the decision space, formulated as 
% \begin{equation}
% \begin{aligned}
%     & L^d_{i,\text{adapt}} = \mathcal{L}(D^P\circ U^P(\{F^k_{iP}~|~\forall k\}),~\text{GT}^P) \\
%     & L^d_{i,\text{revert}} = \left(\mathcal{L}(D^{l_i}\circ U^{l_i}(\{F^k_{Pi}~|~\forall k\}),~\text{GT}^i) + \mathcal{L}(D^{l_i}\circ U^{l_i}(\{F^k_{ii}~|~\forall k\}),~\text{GT}^i)\right)
% \end{aligned}
% \end{equation}
% We use scaling factors $\lambda^f_{\text{adapt}}$, $\lambda^f_{\text{revert}}$, $\lambda^d_{\text{adapt}}$, and $\lambda^d_{\text{revert}}$ to balance the importance between adaptation and reversion, as well as between feature and decision space alignment, ending up with the final loss function for local model $i$ as follow
% \begin{equation}
%     L_i = \lambda^f_{\text{adapt}} L^f_{i,\text{adapt}} + \lambda^f_{\text{revert}} L^f_{i,\text{revert}} + \lambda^d_{\text{adapt}} L^d_{i,\text{adapt}} + \lambda^d_{\text{revert}} L^d_{i,\text{revert}}
% \end{equation}

\subsection{Adapter and Reverter Architecture}

To bridge the domain gap between heterogeneous agents, we propose a flexible architecture for both the adapter $\upphi$ and reverter $\uppsi$. This architecture addresses three main sources of domain gap caused by agent heterogeneity, as identified by~\cite{xu2023bridging}: spatial resolution, feature patterns, and channel dimensions. Our design employs simple linear interpolation for spatial resolution alignment, three ConvNeXt layers \citep{liu2022convnet} with hidden channel dimension $C_\text{hidden}$ for feature pattern alignment, and two additional convolutional layers for channel dimension alignment (input: $C_\text{in}$ $\rightarrow$ $C_\text{hidden}$, output: $C_\text{hidden}$ $\rightarrow$ $C_\text{out}$).

The complete architecture flow is: input ($W_\text{in}, H_\text{in}, C_\text{in}$) $\rightarrow$ spatial resolution alignment ($W_\text{out}, H_\text{out}, C_\text{in}$) $\rightarrow$ input alignment ($W_\text{out}, H_\text{out}, C_\text{hidden}$) $\rightarrow$ feature pattern alignment ($W_\text{out}, H_\text{out}, C_\text{hidden}$) $\rightarrow$ output alignment ($W_\text{out}, H_\text{out}, C_\text{out}$) $\rightarrow$ output ($W_\text{out}, H_\text{out}, C_\text{out}$). This design enables effective mapping between local feature space $F_i$ and protocol feature space $F_P$, irrespective of differences in spatial resolution, feature patterns, or channel dimensions.

Note that this high-level architecture is flexible and open to various implementations. In Section \ref{sec:ablation}, we evaluate alternative approaches for feature pattern alignment, demonstrating our framework's flexibility across different specific implementations.

% To bridge the domain gap between heterogeneous agents, we propose a flexible architecture for both the adapter $\upphi_i$ and reverter $\uppsi_i$. This architecture addresses three main sources of domain gap caused by agent heterogeneity, as identified by Xu et al. \cite{xu2023bridging}: spatial resolution, feature patterns, and channel dimensions.
% Our architecture comprises three key components:

% \textbf{Spatial Resolution Alignment:} Simple linear interpolation adapts features to a common spatial resolution.

% \textbf{Feature Pattern Alignment:} ConvNeXt layers \cite{liu2022convnet} with hidden channel dimension $C_\text{hidden}$ align discrepancies in feature patterns.

% \textbf{Channel Dimension Alignment:} Two convolutional layers handle varying channel dimensions of input: $C_\text{in}$ $\rightarrow$ $C_\text{hidden}$

% Input adaptation: $C_\text{in}$ $\rightarrow$ $C_\text{hidden}$
% Output adaptation: $C_\text{hidden}$ $\rightarrow$ $C_\text{out}$


% The complete architecture flow is:
% Input ($C_\text{in}$) $\rightarrow$ Spatial Resolution Alignment $\rightarrow$ Input Adaptation $\rightarrow$ ConvNeXt Layers $\rightarrow$ Output Adaptation $\rightarrow$ Output ($C_\text{out}$)
% This design enables effective mapping between local feature space $F_i$ and protocol feature space $F_P$, irrespective of differences in spatial resolution, feature patterns, or channel dimensions.
% Notably, this high-level architecture is flexible and open to various implementations. In Section \ref{sec:ablation}, we evaluate alternative approaches for feature pattern alignment, such as using a single convolution layer or a self-attention layer. These experiments demonstrate the robustness of our framework across different specific implementations. We believe that further optimization of each sub-component presents a promising direction for future research.


==> sec/3_methodoloy_bk.tex <==

\section{Methodology}

% Existing mid-fusion collaborative perception algorithm uses the BEV feature of each agents directly for fusion, which challenged by multiple 
% \subsection{Preliminary}

% \noindent \textbf{Definition of Heterogeneous Collaborative Model and Agents:} Collaborative-perception-guided autonomous driving model can be heterogeneous in multiple aspects including: 
% \begin{itemize}
%     \item Input modalities, which requires heterogeneous encoders.
%     \item Downsteam tasks, which requires heterogeneous decoders and evaluation metric
%     \item Fusion Models
%     \item Communication Bandwidth Limitation, which results in heterogeneous feature resolution and dimensions.
% \end{itemize}
% \XG{Consider list a couple of existing collaborative models and show the heterogenity between them. Current we have it on Table \ref{tab:task_agnostic}, but seems like it is too far away from the methology section and it only contains three models}

% \noindent\textbf{Definition of Heterogeneous Collaborative Perception}

% \noindent Consider a local collaborative model $l_i$, it usually consists an encoder \( E^{l_i} \), a collaborative fusion layer $\U^{l_i}$, and a decoder $D^{l_i}$. We further consider that, in collaborative perception scenario, a total of $K$ agents are ready for collaboration and each receives the input data $I^{l_i}_k$ where $k \in [1, K]_\mathbb{Z}$. Now for annotation simplicity, we assume all model receives the same number of agents. This assumption does not lose generality for heterogeneous agent numbers.

% By receiving the input data $I^{l_i}_k$, encoder $E^{l_i}$ maps it to the BEV feature \( F^{l_i}_k \). Then, The BEV feature \( F^{l_i}_k \) of each agent is broadcast to other agents within the collaborative distance $d$, the maximum distance for two agents to collaborate. Next, The collaborative fusion layer \( \U^{l_i} \) gathers and fuses the BEV features from all collaborating agents, resulting in the fused BEV feature \( F'^{l_i} \).  Finally, the decoder \( D^{l_i} \) decodes the fused BEV feature \( F'^{l_i} \) to the final model output \( O^{l_i} \). This procedure is mathematically formulated as follows:

% \[
% \scalebox{1}{%
% \begin{minipage}{\columnwidth}
% \begin{equation}
% \begin{aligned}
%                             & O^{l_i}_k = D^{l_i}(F'^{l_i}_k),\quad \text{for}~k\in [1,K]_{\mathbb{Z}} \\
%     \text{where}\quad       & F'^{l_i}_{1:K} = \U^{l_i}(F^{l_i}_{1:K}),\\
%                             & F^{l_i}_k = E^{l_i}(I^{l_i}_k),\quad \text{for}~k\in [1,K]_{\mathbb{Z}} 
% \end{aligned}
% \end{equation}
% \end{minipage}
% }
% \]


% \[
% \scalebox{1}{%
% \begin{minipage}{\columnwidth}
% \begin{equation}
% \begin{aligned}
%                             & \mathbf{O}^{l_i}_k = \D^{l_i}(\F'^{l_i}_k),\quad \text{for}~k\in [1,K]_{\mathbb{Z}} \\
%     \text{where}\quad       & \F'^{l_i}_{1:K} = \U^{l_i}(\F^{l_i}_{1:K}),\\
%                             & \F^{l_i}_k = \E^{l_i}(\I^{l_i}_k),\quad \text{for}~k\in [1,K]_{\mathbb{Z}} 
% \end{aligned}
% \end{equation}
% \end{minipage}
% }
% \]


% \noindent Collaborative-perception-guided autonomous driving model can be heterogeneous (abbreviate as hetero) in multiple aspects including: 
% \begin{itemize}
%     \item Input modality, results in hetero encoders $E^{l_i}$
%     \item Fusion method, results in hetero fusion Models $\U^{l_i}$
%     \item Downstream tasks, results in hetero decoders $D^{l_i}$
%     \item Communication bandwidth limitation, results in hetero feature $F^{l_i}_{1:K}$ representation including resolution and dimensions.
% \end{itemize}
% \XG{Consider list a couple of existing collaborative models and show the heterogenity between them. Current we have it on Table \ref{tab:task_agnostic}, but seems like it is too far away from the methology section and it only contains three models}

% The aformentioned heterogenity results in hetero representation of the BEV feature, which is the core communicative data for collaborative perception. In the collaborative perception scenario, two models are named hetero models if they contains hetero components, or result in hetero feature representations; two agents are named hetero agents if they are equipped with hetero models.

% \noindent\textbf{Collaborative-partitioned Set and covering Set: \XG {This section is Deprecate }}

% \noindent For clearly illustrate our proposed pipeline, we introduce the concept of Collaborative-partitioned Set and Collaborative-covering Set. Consider the agent set $[1,K]_\mathbb{Z}$ equipped with their corresponding models. We say $S_{\text{par}} = \bigcup_{i=k}^n A_k$ is a partitioned set if and only if 
% \begin{equation}
% \begin{aligned}
%     & 1.\quad A_k \neq \emptyset\quad\text{for all}~k,~\text{and} \\
%     & 2.\quad A_k \cap A_{k'} = \emptyset\quad\text{for all}~k \neq k'
% \end{aligned}
% \end{equation}
% and $A_k$ is a collaborative partition. We say that all agents in the same collaborative partition are collaborative. By this definition, all agents belong and only belong to a single collaborative partition.

% By this definition, traditional single-agent perception model is a partitioned set with only one element in each partition, $i.e.$ $|A_k|=1$ for all $k$, which has sub-optimal model performance. Homogeneous collaborative perception model assumes there is only one partition containing all elements $i.e.$ $A = S_\text{par}$, which is a over-simplied assumption since two model may not be collaborative due to the model or data heterogeneity. Existing heterogeneous collaborative models following the most general definition of partitioned set such that each partition may contain multiple elements. Xu \emph{et. al.}~\cite{xu2023bridging} use paired adapters to aligned the bev feature of two hetero models. Lu \emph{et. al.}~\cite{lu2024an} introduced backward alignment training strategy to aligned the bev features of hetero models. Besides their effectiveness, their 

% collaborative 



\subsection{Overview}

Our proposed pipeline aims to perform collaboration among existing heterogeneous collaborative agents without sharing the models' details or downstream task information. To be specific, we add two extra step between the \Eqref{eq:encoding} and \Eqref{eq:fusion}, which are called Adaptation and Reversion. We introduce an local adapter $\upphi_i$ and local reverter $\uppsi_i$ pair for each agent, where $\upphi_i$ maps local BEV feature $F_i$ to an unified BEV feature representation. We name the unified BEV feature as protocol feature with notation $F_P$, and we name the local BEV feature $F_i$ that is adapted to protocol feature representation as adapted feature with notation $F_{iP}$. This step is formulated as,
\begin{equation}
    \text{Adaptation:} \quad F_{iP} = \upphi_i(F_i), \quad \forall i \in \{1, 2, \ldots, N\} \label{eq:adaptation}
\end{equation}
Then, the adapted features of all heterogeneous agents $i$ are broadcast to other agents $j$ within a collaborative distance $d$. Each other agent $j$ receive the adapted features and use their own local reverter $\uppsi_j$ to map the adapted features to its own local feature representation, which are named reverted features with notation $\{F_{ij}\ |\ i\neq j\}$. This step is formulated as,
\begin{equation}
    \text{Reversion:} \quad F_{ij} = \uppsi_j(F_{iP}), \quad \forall i, j \in \{1, 2, \ldots, N\} \label{eq:reversion}
\end{equation}
With the modified \Eqref{eq:fusion}: $F'_j = U_j(\{F_{kj} ~|~\mathcal{N}(j, k) \leq d\}), \quad \forall j \in \{1, 2, \ldots, N\}$, the adaptation and reversion step seamlessly integrated to standard hetero collaborative perception pipeline resulting our proposed MasCo.

To train the unified BEV feature representation as well as the local adapter and reverter pairs, we propose \textbf{Collaborative Adaptation} (\Secref{sec:collab_adapt}) \XG{May need to change a name to not confused with the adaptation process.} As shown in Fig.~\ref{figure:pipeline}, before \textbf{Collaborative Adaptation} (A), hetero agents are performing multiple tasks individually with no ability to collaborate with other agents, which results in sub-optimal performance. After \textbf{Collaborative Adaptation} (C), hetero agents are collaborative and result in a performance boost.

% \noindent \textbf{MASCO Inference Pipeline:} Consider $K$ local agents $l_i$, where $i\in[1,K]_{\mathbb{Z}}$ indicates the heterogeneous agent index, with each taking $I^{l_i}$ as input. Intermediate BEV feature of each local agent $F^{l_i}$ is retrieved by $F^{l_i} = E^{l_i}(I^{l_i})$. Considering the heterogeneity of the local BEV feature representation, we firstly learn a mapping function $\upphi^{l_i}$ for each local model $l_i$, we name it local adapter, that maps local BEV feature $F^{l_i}$ to an unified BEV feature representation. We name this unified BEV feature as protocol feature with notation $F^P$. We call the local BEV feature $F^{l_i}$ that is adapted to protocol feature representation as adapted feature with notation $F^{l_i\rightarrow P}$. Then, the adapted features from all heterogeneous agents are broadcast to other agents within a collaborative distance \( d \)\XG{Thinking of drawing a figure to illustrate this process}. Other agents receive the adapted features and use another mapping function $\uppsi^{l_i}$, we name it local reverter, that maps the adapted features to their own local feature representation, which we called reverted feature with notation $F^{l_i\rightarrow P \rightarrow l_j},i\neq j$, where $l_i$ and $l_j$ refers to the local model $i$ and $j$ respectively. Then, all reverted features from other agents $\{F^{l_i\rightarrow P \rightarrow l_j},i\neq j\}$ are transformed to local agent coordinate and are passed into the local fusion model $\U^{l_i}$ along with its own local BEV feature $F^{l_i}$ to retrieve the fused BEV feature $F'^{l_i}$ by $F'^{l_i} = \U^{l_i}(\mathcal{S}^{l_i})$, where $\mathcal{S}=\{F^{l_i\rightarrow P \rightarrow l_j},i\neq j\}\cup F^{l_i}$. Finally, the fused BEV feature $F'^{l_i}$ of each local agent is passed into the local decoder $D^{l_i}$ to perform local task by $O^{l_i}=D^{l_i}(F'^{l_i})$. This inference pipeline is summarized in \Algref{alg:inference}. Since we assume $E^{l_i},\U^{l_i},D^{l_i}$ are given by each local agent, for each local agent $l_i$, we only required to train an local adapter $\upphi^{l_i}$ and a local reverter $\uppsi^{l_i}$.

% \begin{algorithm}[h]
% %\small
% \caption{MASCO Inference Pipeline}
% \label{alg:inference}
% \begin{algorithmic}[1]
% \State \textbf{Prepare} $\upphi^{l_i}$, $\uppsi^{l_i}$, $I^{l_i},E^{l_i},\U^{l_i},D^{l_i} \text{ for all } i$
% \State \textbf{Initialize} $d$
% \For{all $i$}
%     \State $F^{l_i} \leftarrow E^{l_i}(F^{l_i})$ \hfill \comment{Encode features using the local encoder}
%     \State $F^{l_i\rightarrow P} \leftarrow \upphi^{l_i}(F^{l_i})$ \hfill \comment{Use local adapter to retrieve adapted features}
%     \State Boardcast $F^{l_i\rightarrow P}$ to other local agents within collaborative distance $d$.
% \EndFor
% \For{all $i$}
%     \State Receive $\{F^{l_j\rightarrow P},\ j \neq i\}$ from other local agents
%     \State $\mathcal{S}^{l_i} \leftarrow \{F^{l_i}\}$ \hfill \comment{Initialize feature set for fusion}
%     \For{all $\{j,\ j\neq i\}$}
%         \State $F^{l_i\rightarrow P\rightarrow l_j} \leftarrow \uppsi^{l_j}(F^{l_j\rightarrow P})$ \hfill \comment{Use local reverters to retrieve reverted features}
%         \State $F^{l_i\rightarrow P\rightarrow l_j} \leftarrow \text{Transform}^{l_i}(F^{l_i\rightarrow P\rightarrow l_j})$ \hfill \comment{Transform the features to local coordinate}
%         \State $\mathcal{S}^{l_i} \leftarrow \mathcal{S}^{l_i}\cup \{F^{l_i\rightarrow P\rightarrow l_j}\}$ \hfill \comment{Aggregate reverted features}
%     \EndFor
%     \State $F'^{l_i} \leftarrow \U^{l_i}(\mathcal{S}^{l_i})$ \hfill \comment{Fuse all features to get a fused BEV feature}
%     \State $O^{l_i} \leftarrow D^{l_i}(F'^{l_i})$ \hfill \comment{Perform local downstream task}
% \EndFor
% \end{algorithmic}
% \end{algorithm}





% \begin{algorithm}[t]
% %\small
% \caption{MASCO Inference Pipeline}
% \label{alg:inference}
% \begin{algorithmic}[1]
% \State \textbf{Prepare} $\{\upphi^i, \uppsi^i, \I^i, \E^i, \U^i, \D^i\} \text{ for all } i$
% \State \textbf{Initialize} $d$
% \For{all $i$}
%     \State $\F^i \leftarrow \E^i(\F^i)$ \hfill \comment{Encode features using the local encoder}
%     \State $\F^{iP} \leftarrow \upphi^i(\F^i)$ \hfill \comment{Use local adapter to retrieve adapted features}
%     \State Boardcast $\F^{iP}$ to other local agents within collaborative distance $d$.
% \EndFor
% \For{all $j$}
%     \State Receive $\{\F^{iP},\ i \neq j\}$ from other local agents
%     \State $\mathcal{S}^j \leftarrow \{\F^j\}$ \hfill \comment{Initialize feature set for fusion}
%     \For{all $\{i,\ i\neq j\}$}
%         \State $\F^{ij} \leftarrow \uppsi^i(\F^{iP})$ \hfill \comment{Use local reverters to retrieve reverted features}
%         \State $\F^{ij} \leftarrow \text{Transform}^j(\F^{ij})$ \hfill \comment{Transform the features to local coordinate}
%         \State $\mathcal{S}^j \leftarrow \mathcal{S}^j \cup \{\F^{ij}\}$ \hfill \comment{Aggregate reverted features}
%     \EndFor
%     \State $\F'^j \leftarrow \U^j(\mathcal{S}^j)$ \hfill \comment{Fuse all features to get a fused BEV feature}
%     \State $\mathbf{O}^j \leftarrow \D^j(\F'^j)$ \hfill \comment{Perform local downstream task}
% \EndFor
% \end{algorithmic}
% \end{algorithm}










% Define a custom column type to ensure consistent spacing
% \newcolumntype{L}{>{\raggedright\arraybackslash}m{7cm}}
% \newcolumntype{C}{>{\raggedright\arraybackslash}m{2cm}}


% \begin{table}[h]
%     \centering
%     \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{CL}
%         \hline
%         \textbf{Symbol} & \textbf{Description} \\ \hline
%         $P$ & Protocol model \\ \hline
%         $M_i$ & the $\ith{k}$ model \\ \hline
%         $*^P$ & * of the protocol model, $\text{*} \in \{E, \text{U}, \text{D}, \text{O}, \text{L}, \text{GT}\}$ \\ \hline
%         $*^{M_i}$ & * of the $\ith{k}$ model, $\text{*} \in \{E, \upphi, \uppsi, \text{U}, \text{D}, \text{O}, \text{L}, \text{GT}\}$ \\ \hline
%         $E$ & Encoder \\ \hline
%         $\upphi$ & Adapter \\ \hline
%         $\uppsi$ & Reverter \\ \hline
%         $U$ & Collaborative fusion layer \\ \hline
%         $D$ & Decoder \\ \hline
%         $O$ & Model output \\ \hline
%         $GT$ & Ground truth label \\ \hline
%         % $\mathcal{L}$ & Loss function \\ \hline
%         % $L$ & Calculated loss \\ \hline
%         % $\lambda^{\rightarrow P}$ & Scaling factor for  \\ \hline
%         % $\lambda^{\rightarrow M_i}$ & scaling factor for each loss to balance the importance between adaptation and reversion. \\ \hline
%         $I^P_k$ & Input data of the protocol model for the $\ith{k}$ agent  \\ \hline
%         $I^{M_i}_k$ & Input data of the $\ith{k}$ model for the $\ith{k}$ agent \\ \hline
%         $F^P_k$ & BEV feature of the protocol model for the $\ith{k}$ agent \\ \hline
%         $F^{M_i}_k$ & BEV feature of the $\ith{k}$ model for the $\ith{k}$ agent \\ \hline
%         $F^{M_i \rightarrow P}_k$ & BEV feature of the $\ith{k}$ model for the $\ith{k}$ agent mapped to the protocol domain \\ \hline
%         $F^{M_i \rightarrow P \rightarrow M_j}_k$ & BEV feature of the $\ith{k}$ model for the $\ith{k}$ agent mapped to the protocol domain and then to model $j$'s domain \\ \hline
%         $F^{P \rightarrow M_j}_k$ & BEV feature of the protocol model for the $\ith{k}$ agent mapped to model $j$'s domain \\ \hline
%         $d$ & Collaborative distance: the maximum distance for two agents to collaborate \\ \hline
%         $K$ & Number of agents for collaborative perception \\ \hline
%         $N$ & Number of local models \\ \hline
%     \end{tabular}}
%     \caption{List of important notations. Note that this table is not a full list of notations.}
%     \label{tab:notations}
% \end{table}

\begin{figure*}[t]
\includegraphics[width=\textwidth]{Figures/pipeline_v2.pdf}
\caption{}
\label{figure:pipeline}
\end{figure*}


\subsection{Collaborative Adaptation}
\label{sec:collab_adapt}
\subsubsection{Training Protocol Network}

The first step is to learn an unified BEV feature distribution, in our case, training a protocol network. Training protocol networks is the same as training an ordinary collaborative perception model, following \Eqrefs{eq:encoding}{eq:fusion}{eq:decoding}.  We use $E_P,U_P,D_P$ to denote the protocol encoder, fusion model, and decoder, respectively. We use $I_P, F_P,F'_P,O_P$ to denote the input data, BEV feature, fused BEV feature, and final output of the protocol model, respectively. Same as local models, protocol model is not restricted to any specific model or downstream task.

% We use $*_P$ to denote the protocol feature or protocol model, where $*\in\{E,U,D,I,F,F',O\}$. 




% \[
% \scalebox{1}{%
% \begin{minipage}{\columnwidth}
% \begin{equation}
% \begin{aligned}
%                             & O^P_k = D^P(F'^P_k),\quad \text{for}~k\in [1,K]_{\mathbb{Z}} \\
%     \text{where}\quad       & F'^P_{1:K} = U^P(F^P_{1:K}), \\
%                             & ~F^P_k = E^P(I^P_k),\quad \text{for}~k\in [1,K]_{\mathbb{Z}}
% \end{aligned}
% \end{equation}
% \end{minipage}
% }
% \]
% where $I^P$ refers to the input of protocol model. $E^P$, $U^P$, and $D^P$ refers to the encoder, fusion model, and decoder of protocol model respectively. 





\subsubsection{Training Local Adapters and Reverters}

Here we introduce a new notation $\mathcal{X}=\{\mathbf{x}^1, \mathbf{x}^2, \hdots, \mathbf{x}^K\}$ to denote a set of physical world information, where $K$ denotes the total number of physical world information, and a modality transformation function $\mathcal{T}:\mathcal{X} \to I$ that transforms physical world information to sensor data of given modality. For example, in the autonomous driving scenario, by letting $\mathbf{x}$ to be the physical world information surrounded by the ego vehicle, $\mathcal{T}$ to be the matrix of six surround-view RGB cameras, then $I$ would be the six RGB images captured by the cameras.

% Given local model $i$, we aim to train a local adapter $\upphi_i$ and reverter $\uppsi_i$ pair, so all model parameters of the local model $i$ and protocol models $P$ are fixed, except for $\upphi_i$ and $\uppsi_i$. 

Given a local model $i$, protocol model $P$, and a set of physical world information $\mathcal{X}=\{\mathbf{x}^1, \mathbf{x}^2, \hdots, \mathbf{x}^K\}$, we have $I^k_i = \mathcal{T}_i(\mathbf{x}^k)$ to be the input of local model $i$ and $I^k_P = \mathcal{T}_P(\mathbf{x}^k)$ to be the input of protocol model $P$, where $\mathcal{T}_i$ and $\mathcal{T}_P$ denote the sensor modalities of the local model $i$ and protocol model, respectively. Consider local BEV feature $F^k_i=E_i(\mathcal{T}_i(\mathbf{x}^k))$ and protocol BEV feature $F^k_P=E_P(\mathcal{T}_P(\mathbf{x}^k))$, there is a domain gap between them due to the heterogeneity of sensor modalities $\mathcal{T}_i$ and $\mathcal{T}_P$ as well as the encoders $E_i$ and $E_iP$. To bridge this domain gap, \XG{We need to discuss in later section that why finding adapter instead of learning a new encoder is a better way}, we map the local BEV feature $F^k_i$ from its representation to the protocol feature representation by finding a local adapter $\upphi_i$ such that 
\begin{equation}
    \upphi_i = \argmin_{\upphi_i} \sum_{k} \text{Norm}_{\text{adapt}}(F^k_{iP}, F^k_P) \quad \text{where} \quad F^k_{iP} = \upphi_i(F^k_i)
\end{equation}
Simliar, we aim to find a reverter $\uppsi_i$ that maps the protocol BEV feature $F^k_P$ from the protocol representation to the local feature representation, $i.e.$, $\uppsi_i(F^k_P)$. Additionally, since $F^k_{iP}$ is also in the protocol representation, we also align $\uppsi_i(F^k_{iP})$ with $F^k_i$ for stronger supervision signal.
% \begin{equation}
% \resizebox{0.9\textwidth}{!}{$
%     \uppsi_i = \argmin_{\uppsi_i} \sum_{k} \left(L_{\text{revert}}(F^k_{Pi}, F^k_i) + L_{\text{revert}}(F^k_{ii}, F^k_i)\right) \quad \text{where} \quad F^k_{Pi} = \uppsi_i(F^k_P),\ F^k_{ii} = \uppsi_i(F^k_{iP})
% $}
% \end{equation}
\begin{equation}
\begin{aligned}
    & \uppsi_i = \argmin_{\uppsi_i} \sum_{k} \left(\text{Norm}_{\text{revert}}(F^k_{Pi}, F^k_i) + \text{Norm}_{\text{revert}}(F^k_{ii}, F^k_i)\right) \\
    \text{where} \quad &   F^k_{Pi} = \uppsi_i(F^k_P),\ F^k_{ii} = \uppsi_i(F^k_{iP})
\end{aligned}
\end{equation}

\noindent \textbf{Aligning Intermediate Feature Space:} Given local model $i$, We firstly align $(F^k_{iP}, F^k_P)$, $(F^k_{Pi}, F^k_i)$, and $(F^k_{ii}, F^k_i)$ pairs for all $k$ by using \( L2 \)-norm to directly align their feature space, $i.e.$, 
% \begin{equation}
% \resizebox{0.9\textwidth}{!}{$
%     L^f_{i,\text{adapt}} = \frac{1}{K} \sum_{k} \text{L2Loss}(F^k_{iP}, F^k_P),\quad L^f_{i,\text{revert}} = \frac{1}{K} \sum_{k} \left(\text{L2Loss}(F^k_{Pi}, F^k_i) + \text{L2Loss}(F^k_{ii}, F^k_i)\right)
% $}
% \end{equation}
\begin{equation}
\begin{aligned}
    & L^f_{i,\text{adapt}} = \frac{1}{K} \sum_{k} \|F^k_{iP}, F^k_P\|_2 , \\
    & L^f_{i,\text{revert}} = \frac{1}{K} \sum_{k} \left(\|F^k_{Pi}, F^k_i\|_2 + \|F^k_{ii}, F^k_i\|_2\right)
\end{aligned}
\end{equation}


\noindent \textbf{Aligning Decision Space:} Under the case where $\mathcal{T}_i$ and $\mathcal{T}_P$ are hugely different, such as rgb images and lidar point clouds, the resulting large gap between the intermediate feature representations. \help{Please take a look at the difference between \underline{aligning feature space} and \underline{aligning decision space}. I am looking for a mathematical explanation of why we need aligning decision space. The intuition is that under the case where $\min_{\upphi_i} L_{\text{adapt}}(F_{iP}, F_P)$ cannot be 0, we should prioritize to minimize the final output result. \textbf{OR}, we can think about this in distillation way, where aligning decision space is \underline{output distillation} while aligning feature space is \underline{feature distillation}}.

In this case, it is neither possible nor necessary to find a $\upphi_i$ such that $F^k_{iP}$ to be the same as $F^k_P$. 

% However, because $F^k_i$ and $F^k_{iP}$ share the same physical world information $\mathbf{x}^k$ for all $k$, the downstream task outputs $D_P\circ U_P(\{F^1_{iP}, F^2_{iP}, \hdots, F^K_{iP}\}))$ should be equal to $D_P\circ U_P(\{F^1_P, F^2_P, \hdots, F^K_P\}))$. Similarly, the downstream task outputs $D_i\circ U_i(\{F^1_{ii}, F^2_{ii}, \hdots, F^K_{ii}\}))$ should be equal to $D_i\circ U_i(\{F^1_i, F^2_i, \hdots, F^K_i\}))$. 

However, because $F^k_i$ and $F^k_{iP}$ share the same physical world information $\mathbf{x}^k$ for all $k$, the downstream task outputs of the adapted local features $D_P\circ U_P(\{F^k_{iP}~|~\forall k\})$ has the same ground truth labels $\text{GT}_P$ as the output of protocol features $D_P\circ U_P(\{F^k_P~|~\forall k\})$. Similarly, the downstream task outputs of the reverted local features $D_i\circ U_i(\{F^k_{ii}~|~\forall k\}))$, reverted protocol feature $D_i\circ U_i(\{F^k_{Pi}~|~\forall k\})$, and the original local features $D_i\circ U_i(\{F^k_i~|~\forall k\}))$ has the the same ground truth labels $\text{GT}_i$. 



To this end, we propose additional loss to align the features in the decision space, formulated as 
% \[
% \scalebox{1}{%
% \begin{minipage}{\columnwidth}
% \begin{equation}
% \begin{aligned}
%                         & L_d = \lambda_d^{\rightarrow P} L_d^{\rightarrow P} + \lambda^{\rightarrow l_i}L^{\rightarrow l_i} \\
%     \text{where}\quad   & L_d^{\rightarrow P} = \mathcal{L}(D^P\circ U^P(\{F^{l_i\rightarrow P}\}),~\text{GT}^P) \\
%                         & L_d^{\rightarrow l_i} = \mathcal{L}(D^{l_i}\circ U^{l_i}(\{F^{l_i\rightarrow P\rightarrow l_i}\}),~\text{GT}^{l_i})
% \end{aligned}
% \end{equation}
% \end{minipage}
% }
% \]

\begin{equation}
\begin{aligned}
    & L^d_{i,\text{adapt}} = \mathcal{L}(D^P\circ U^P(\{F^k_{iP}~|~\forall k\}),~\text{GT}^P) \\
    & L^d_{i,\text{revert}} = \left(\mathcal{L}(D^{l_i}\circ U^{l_i}(\{F^k_{Pi}~|~\forall k\}),~\text{GT}^i) + \mathcal{L}(D^{l_i}\circ U^{l_i}(\{F^k_{ii}~|~\forall k\}),~\text{GT}^i)\right)
\end{aligned}
\end{equation}
We use scaling factors $\lambda^f_{\text{adapt}}$, $\lambda^f_{\text{revert}}$, $\lambda^d_{\text{adapt}}$, and $\lambda^d_{\text{revert}}$ to balance the importance between adaptation and reversion, as well as between feature and decision space alignment, ending up with the final loss function for local model $i$ as follow
\begin{equation}
    L_i = \lambda^f_{\text{adapt}} L^f_{i,\text{adapt}} + \lambda^f_{\text{revert}} L^f_{i,\text{revert}} + \lambda^d_{\text{adapt}} L^d_{i,\text{adapt}} + \lambda^d_{\text{revert}} L^d_{i,\text{revert}}
\end{equation}




% We denote $\upphi_i(F_i)$ as $F_{iP}$ and we 
% use an \( L2 \)-norm to align $F_P$ and $F_{iP}$, $i.e.$
% \begin{equation}
%     L^f_{i,P} = \text{L2Loss}(F_{iP}, F_P)
% \end{equation}


% With $I_i$ being the model input, we have local BEV feature $F_i = E_i(I_i)$. By letting the protocol take the same input $I_i$ to get $F_P = E_P(I_P)$, we except $F_i$ and $F_P$ to represent the same physical-world information but in heterogeneous feature representation. To bridge this domain gap, we map $F_i$ to the protocol BEV feature representation to get $F_{iP}=\upphi_i(F_i)$. We use an \( L2 \)-norm to align $F_P$ and $F_{iP}$, $i.e.$
% \begin{equation}
%     L^f_{i,P} = \text{L2Loss}(F_{iP}, F_P)
% \end{equation}
% To train the reverter $\uppsi_i$, we use it to map both $F_P$ and $F_iP$ to the local BEV feature representation to get $F_{Pi}$ and $F_{ii}$ respectively. We also use an \( L2 \)-norm to align them with the original local BEV feature $F_i$, $i.e.$
% \begin{equation}
%     L^f_{i,P} = \text{L2Loss}(F_{Pi}, F_i) + \text{L2Loss}(F_{ii}, F_i)
% \end{equation}
% Note that in this procedure, we fix the gradient for \( \uppsi_i \) while learning $\upphi$ to avoid \XG{learning bijective function? maybe some citations?} We use scaling factors $\lambda^f_{\text{adapt}}$ and $\lambda^f_{\text{revert}}$ to balance the importance between adaptation and reversion, and the final loss of local model $i$ for aligning intermediate feature space is
% \begin{equation}
%     L^f = \lambda^f_{\text{adapt}} L^f_P + \lambda^f_{\text{revert}} L^f_i \\
% \end{equation}

% For each local model $l_i$, an adapter \(\upphi^{l_i}\) maps the BEV feature \(F^{l_i}\) from the local model \(l_i\)'s domain to the BEV feature \(F^{l_i \rightarrow P}\) in the protocol domain. A reverter \(\uppsi^{l_i}\) maps the BEV features \(F^P\) and \(F^{l_i \rightarrow P}\) from the protocol model's domain to the BEV features \(F^{P \rightarrow l_i}\) and \(F^{l_i \rightarrow P \rightarrow l_i}\) in the model \(l_i\)'s domain. Mathematically, this can be formulated as follows for all $i$:
% \[
% \scalebox{1}{%
% \begin{minipage}{\columnwidth}
% \begin{equation}
% \begin{aligned}
%                             & F^{l_i\rightarrow P\rightarrow l_i} = \uppsi^{l_i}(F^{l_i\rightarrow P}) \\
%                             & F^{P\rightarrow l_i} = \uppsi^{l_i}(F^P) \\
%     \text{where}\quad       & F^{l_i\rightarrow P} = \upphi^{l_i}(F^{l_i}) \\
% \end{aligned}
% \end{equation}
% \end{minipage}
% }
% \]

% where \(N\) denotes the total number of local models.



 % To align \( F^{l_i \rightarrow P} \) with the protocol domain, and align \( F^{P \rightarrow l_i} \) and \( F^{l_i \rightarrow P \rightarrow l_i} \) to the local model \( l_i \)'s domain, we use an \( L2 \)-norm loss function, formulated as follows:

% \XG{Padding of visible range for feature space alignment}

% \[
% \scalebox{1}{%
% \begin{minipage}{\columnwidth}
% \begin{equation}
% \begin{aligned}
%                         & L_f = \lambda_f^{\rightarrow P} L_f^{\rightarrow P} + \lambda^{\rightarrow l_i}L^{\rightarrow l_i} \\
%     \text{where}\quad   & L_f^{\rightarrow P} = \text{L2Loss}(F^{l_i\rightarrow P}, F^P) \\
%                         & L_f^{\rightarrow l_i} = \text{L2Loss}(F^{P\rightarrow l_i}, F^{l_i}) + \text{L2Loss}(F^{l_i\rightarrow P\rightarrow l_i}, F^{l_i})
% \end{aligned}
% \end{equation}
% \end{minipage}
% }
% \]








% \XG{Include training with output supervision. The problem of current training strategy is that inferior model (such as camera-based model or very small model) tend to suppress useful information due to its own inferiority.}

% \subsubsection{Perform Collaborative Perception on the Road}

% With all parts trained, we are ready to assemble them and perform collaborative perception with other heterogeneous agents. Consider \( K \) agents on the road, each equipped with their model. We assume all agents are within their collaboration distance for notation simplicity.

% Without loss of generality, consider agent \( k \) equipped with model \( l_i \). It maps its BEV feature \( F^{l_i}_k \) to the protocol domain \( F^{l_i \rightarrow P}_k \) using its local adapter \(\upphi_i\). Then, \( F^{l_i \rightarrow P}_k \) is broadcast to and received by all other agents. The agent receives other agents' BEV features \( F^{M_* \rightarrow P}_{\{1:K\} \backslash \{k\}} \), where \( M_* \) is agnostic, and maps them back to its own BEV feature domain \( F^{M_* \rightarrow P \rightarrow l_i}_{\{1:K\} \backslash k} \). After that, concatenating it with its own BEV feature \( F^{l_i}_k \) and performing collaborative fusion \( U^{l_i} \) and decoding \( D^{l_i} \), we have:
% \[
% \scalebox{1}{%
% \begin{minipage}{\columnwidth}
% \begin{equation}
% \begin{aligned}
%                             & O^{l_i}_k = D^{l_i}(F'^{l_i}_k) \\
%     \text{where}\quad       & F'^{l_i}_k = U^{l_i}(F^{l_i}_k, F^{M_*\rightarrow P\rightarrow M_{i}}_{\{1:K\}\backslash \{k\}})\\
% \end{aligned}
% \end{equation}
% \end{minipage}
% }
% \]

% This completes the collaborative perception process, allowing agents to effectively integrate and utilize the information from other heterogeneous agents within their collaboration range.


\subsection{Adapter and Reverter Architecture}
We use simple linear interpolation to adopt difference in spatial resolution. We use ConvNeXt~\cite{liu2022convnet} layers with channel number $C_\text{hidden}$ to align the discrepancy in feature patterns. We adpot channel number, we add a single convolutional layer with input channels $C_\text{in}$ and output channels $C_\text{hidden}$ before the ConvNeXt layers, and add another convolutional layer with input channels $C_\text{hidden}$ and output channels $C_\text{out}$ after the ConvNeXt layers.
% Besides, we discover that the feature patterns of heterogeneous models can be greatly differ by a simple scaling factor. We multiply the resulting feature by a learnable scaling factor. 


% \XG{develop new architectures or experiment several existing architectures}


==> sec/4_experiments_bk.tex <==
\section{Experiments}

We evaluate the performance of our proposed Model-agnostic and Scalable Collaborative Perception pipeline. One of the key contribution of this work is that our pipeline allow agents with heterogeneous models and tasks to collaborate, requiring no sharing bettween local agents about model or task information. To our knowledge, our pipeline is the first one that achieves this goal. Therefore, to compare with other existing heterogeneous collaborative perception methods, in \Secref{sec:heter_agent}, we simplify the experiments to a single downstream task, 3D object detection. Then, in \Secref{sec:task_agnostic_fusion}, we choose four existing collaborative models with heterogeneous model architectures and downstream tasks to evaluate the performance of our pipeline under the task-agnostic setting. Finally, we conduct some efficiency comparsion in \Secref{sec:eff} and ablation studies in \Secref{sec:ablation}.

\subsection{Experimental Setups}
\label{sec:implementation}
\noindent \textbf{Dataset:} We conduct our experiment on two multi-agent collaborative perception datasets, a simulated dataset OPV2V\cite{xu2022opv2v}, and a real-world dataset V2V4Real\cite{xu2023v2v4real}. For multi-agent collaborative perception, simulated datasets are advantaged by their scale, such as the number of samples and the number of agents in each sample, as well as their diversified input modalities and downstream task annotations. For example, OPV2V contains 11k samples with 4 rgb images and 1 lidar point clouds inputs for each sample. Each sample contains 2-5 agents to performance collaborative perception. It also contains in total of 230k 3D bounding box annotations for the object detection task as well as both static and dynamic object segmentation annotations for the BEV segmentation task. On the other hand, real-world datasets are advantaged by their data realism which more accurately reflects the model performance in the real world. However, real-world datasets  such as V2V4Real only releases 20k samples with lidar point clouds inputs only. Each sample only contains 2 agents for collaborative perception. Besides, V2V4Real release 240K 3D bounding box annotations for 3D object detection task only. For a comprehensive experiments, in \Secref{sec:heter_agent}, we use both the simulated dataset OPV2V and the real-world dataset V2V4Real to compare our pipeline with existing heterogeneous collaborative perception pipeline under the object detection downsteam task. In \Secref{sec:task_agnostic_fusion}, since V2V4Real contains 3D bounding box annotations, we only use OPV2V to evaluate our pipeline under the task-agnostic setting. In \Secref{sec:ablation}, we use V2V4Real to conduct ablation studies, aim to more accurately evaluate the performance of our proposed pipeline in the real-world.



% Adapter $\upphi$ and reverter $\uppsi$ follows similiar model archiectures. We firstly use simple linear interpolation to adapt the difference in spatial resolution. Next, we add a single convolutional layer with input channels $C_\text{in}$ and output channels $C_\text{hidden}$ to adapt channel number. Then we use three layers of ConvNeXt\cite{liu2022convnet} layers with channel number $C_\text{hidden}$ to align the discrepancy in feature patterns. Finally, we add another convolutional layer with input channels $C_\text{hidden}$ and output channels $C_\text{out}$ after the ConvNeXt layers. 

\noindent \textbf{Implementation Details:} We have two different experimental setups for \Secref{sec:heter_agent} under 3D object detection setting and for \Secref{sec:task_agnostic_fusion} under the task agnostic setting. The detailed setups are illustrate within each section. For all experiments except end-to-end train strategy, local models and protocol models are trained for 30 epochs with Adam optimizer~\cite{kingma2014adam}. For end-to-end training, we increased the number of iterations proportionally to the number of agents, i.e., \(\text{Iters}_N = 30N\), where \(N\) represents the number of heterogeneous models. \help{This ensures that each model receives the same level of supervision signals as other methods.} We start the learning rate at $0.001$ and reduce by $0.1$ at the $50\%$ and $83\%$ of the total epochs. We use single NVIDIA RTX A6000 for both model training and inference. Lidar-based models takes approximately 5 hours to train and camera-based models takes approximately 1 day. Local adapter $\upphi$ and local reverter $\uppsi$ are also trained with Adam optimizer but only for 2 epochs. We start the learning rate at $0.01$ and reduced by $0.1$ after the first epoch. Lidar-based models takes about 10 minutes to train and camera-based models takes about 1 hour. We set the loss scaling factor $\lambda^f_\text{adapt} = \lambda^f_\text{revert} = \lambda^d_\text{adapt} = \lambda^d_\text{revert} = 0.5$. For more implementation details, please refer \Secref{sec:heter_agent}, \Secref{sec:task_agnostic_fusion}, and Appendix.


\subsection{Heterogeneous Collaborative Perception For 3D Object Detection}
\label{sec:heter_agent}

\subsubsection{Performance Comparison}


\begin{table*}[h]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{>{\centering\arraybackslash}m{1cm}|>{\centering\arraybackslash}m{2.3cm}|>{\centering\arraybackslash}m{1.2cm}>{\centering\arraybackslash}m{1.2cm}>{\centering\arraybackslash}m{1.2cm}>{\centering\arraybackslash}m{1.2cm}|>{\centering\arraybackslash}m{1.2cm}>{\centering\arraybackslash}m{1.2cm}>{\centering\arraybackslash}m{1.2cm}>{\centering\arraybackslash}m{1.2cm}}
\hline
& & \multicolumn{4}{c|}{AP 30 $\uparrow$} & \multicolumn{4}{c}{AP 50 $\uparrow$} \\ \hline
$\sigma$ & (Hetero) Agents & 1 & 2 & 3 & 4 & 1 & 2 & 3 & 4 \\ \hline

\multirow{5}{*}{0.0}    & Late Fusion     & \textbf{0.902}    & 0.931             & 0.935             & 0.935             & 0.894             & 0.908             & 0.913             & 0.914 \\
                        & Calibrator      & 0.901             & 0.935             & 0.939             & 0.938             & \textbf{0.896}    & 0.914             & 0.916             & 0.920 \\
                        & E2E Training    & 0.899             & 0.973             & 0.978             & 0.986             & 0.885             & 0.967             & 0.977             & 0.980 \\
                        & HEAL            & 0.897             & 0.975             & 0.986             & 0.985             & 0.889             & 0.972             & 0.978             & 0.983 \\
                        & \cellcolor{pink!40} Ours            & \cellcolor{pink!40} \textbf{0.902}    & \cellcolor{pink!40} \textbf{0.981}    & \cellcolor{pink!40} \textbf{0.987}    & \cellcolor{pink!40} \textbf{0.989}    & \cellcolor{pink!40} 0.894             & \cellcolor{pink!40} \textbf{0.977}    & \cellcolor{pink!40} \textbf{0.983}    & \cellcolor{pink!40} \textbf{0.985} \\ \hline

\multirow{5}{*}{0.2}    & Late Fusion     & \textbf{0.900}    & 0.910             & 0.902             & 0.905             & 0.882             & 0.783             & 0.797             & 0.792 \\
                        & Calibrator      & 0.897             & 0.908             & 0.898             & 0.902             & \textbf{0.885}    & 0.778             & 0.800             & 0.791 \\
                        & E2E Training    & \textbf{0.900}    & 0.967             & 0.961             & 0.961             & 0.879             & 0.936             & 0.941             & 0.934 \\
                        & HEAL            & 0.899             & 0.971             & 0.965             & 0.962             & 0.881             & \textbf{0.938}    & 0.940             & 0.940 \\
                        & \cellcolor{pink!40} Ours            & \cellcolor{pink!40} \textbf{0.900}    &  \cellcolor{pink!40} \textbf{0.975}    & \cellcolor{pink!40} \textbf{0.968}    & \cellcolor{pink!40} \textbf{0.968}    & \cellcolor{pink!40} 0.882             & \cellcolor{pink!40} 0.937              & \cellcolor{pink!40} \textbf{0.948}    & \cellcolor{pink!40} \textbf{0.946} \\ \hline





\multirow{5}{*}{0.4}    & Late Fusion     & \textbf{0.888}    & 0.882             & 0.864             & 0.870             & \textbf{0.874}    & 0.639             & 0.614             & 0.617 \\ 
                        & Calibrator      & 0.874             & 0.889             & 0.887             & 0.871             & 0.867             & 0.644             & 0.622             & 0.628 \\ 
                        & E2E Training    & 0.885             & 0.952             & 0.956             & 0.952             & 0.863             & 0.883             & 0.892             & 0.899 \\ 
                        & HEAL            & 0.880             & 0.959             & 0.961             & 0.962             & 0.852             & 0.913             & \textbf{0.915}    & \textbf{0.912} \\ 
                        & \cellcolor{pink!40} Ours            & \cellcolor{pink!40} \textbf{0.888}    & \cellcolor{pink!40} \textbf{0.961}    & \cellcolor{pink!40} \textbf{0.963}    & \cellcolor{pink!40} \textbf{0.966}    & \cellcolor{pink!40} \textbf{0.874}    & \cellcolor{pink!40} \textbf{0.915}    & \cellcolor{pink!40} \textbf{0.915}    & \cellcolor{pink!40} 0.909 \\ \hline
\end{tabular}%
}
\caption{Comparison of different methods under AP 30 and AP 50 metrics on the OPV2V dataset}
\label{tab:results_opv2v}
\end{table*}



In this section, we choose two late fusion methods, vanillan late fusion, and calibrator~\cite{xu2023model}, along with two intermediate fusion methods End-to-end training, and HEAL~\cite{lu2024extensible} for comparing with our heterogeneous collaborative perception pipeline existing pipelines on the 3D object detection task. In collaborative 3D object detection task, using late fusion instead of intermediate fusion is a simple way to alleviate the domain gap. ~\cite{xu2023model} claims that their is still domain gap in late fusion due to the difference of training data and training details among each heterogeneous model, therefore use a calibrator to fill in this domain gap in the decision space. For intermediate fusion, one way to avoid the domain gap is to use end-to-end training. That is, training all heterogeneous models together and let them collaborate during the training stage to fill in the domain gap. ~\cite{lu2024extensible} propose backward alignment technics, train a base network first, then, fix the decoder of the base network and train encoders only to create heterogeneous models. 


% That is, all models share the same decoder. This technics enables new hetero agents to join in, but not scalable \XG{}. 

% However, this training strategy is not only costly in training and usually takes much larger epochs to converge, but also not extensible after finishing training. 

We prepared 12 heterogeneous local models, consisting of six with lidar modality and six with RGB camera modality, as well as one protocol model with lidar modality (Appendix \ref{sec:model_appendix}), following the same training setup as \Secref{sec:implementation}. All lidar agent has visible range  Considering that most samples of OPV2V dataset contains no more than four agents, we only select the first four models for evaluation on the OPV2V dataset. Similiarly, we select the first two models for the V2V4Real dataset since it has two agents for each sample. We use all 12 models to compare the training parameters and estimated train GPU hours in \Secref{sec:eff}.

For the simulated dataset OPV2V, we add Gaussian noise with standard deviation $\sigma = \{0.0, 0.2, 0.4\}$ to simulate the noise in the real-world. As shown in \Figref{tab:results_opv2v}, Late fusion methods (Vanilla late fusion and calibrator) under-perform intermediate fusion as the number of agents goes up. Their performance even goes worse with more agents are joined in, especially in the case of $\sigma = 0.4$. This is because agent 3 and agent 4 are camera agents. The late fusion methods are not robust enough toward the incorrect predictions produced by weaker agents. Comparing with other heterogeneous intermediate fusion pipelines, Our pipeline achieve comparable or even better performance.

\begin{figure*}[h]
\centering
\begin{minipage}{0.45\textwidth}
\centering
\begin{table}[H] % Use H to force the table to stay within the minipage
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{>{\centering\arraybackslash}m{2.1cm}|>{\centering\arraybackslash}m{0.8cm}>{\centering\arraybackslash}m{0.8cm}|>{\centering\arraybackslash}m{0.8cm}>{\centering\arraybackslash}m{0.8cm}}
\hline
 & \multicolumn{2}{c|}{AP 30 $\uparrow$} & \multicolumn{2}{c}{AP 50 $\uparrow$} \\ \hline
Hetero Agents & 1 & 2 & 1 & 2 \\ \hline
Late Fusion & 0.523  & 0.511 & 0.483 & 0.471 \\ 
Calibrator & 0.520  & 0.524 & 0.484 & 0.488 \\ 
E2E Training & 0.513  & 0.612 & 0.473 & 0.598 \\
HEAL & 0.515  & 0.628 & 0.480 & \textbf{0.595} \\ 
\cellcolor{pink!40} Ours & \cellcolor{pink!40} \textbf{0.523}  & \cellcolor{pink!40} \textbf{0.633} & \cellcolor{pink!40} \textbf{0.483} & \cellcolor{pink!40} 0.594 \\ \hline
\end{tabular}%
}
\caption{Comparison of different methods under AP 30 and AP 50 metrics on the V2V4Real dataset}
\label{tab:results_v2v4real}
\end{table}

\end{minipage}\hfill
\begin{minipage}{0.53\textwidth}
\centering
\includegraphics[width=\textwidth]{Figures/efficiency.pdf}
\caption{Training efficiency comparison between our pipeline and existing intermediate heterogeneous collaborative perception pipelines over the number of heterogeneous agents.}
\label{fig:efficiency}
\end{minipage}
\end{figure*}



\Tabref{tab:results_v2v4real} compares the average precision on the V2V4Real dataset. Simliar to the evaluation results on the OPV2V dataset, our pipeline shows prioritized average precision comparing the late fusion methods and competitive results among existing heterogeneous intermediate fusion pipelines.

% We adopt 12 heterogeneous agents, each with lidar point clouds input and PointPillar~\cite{lang2019pointpillars} Encoder, lidar point clouds input and SECOND Encoder~\cite{yan2018second} Encoder, RGB images input and ResNet101 Encoder, as well as RGB images input and EfficientNet-b0 Encoder. All models use pyramid fusion~\cite{lu2024extensible} for collaborative fusion model and  .






% \begin{table}[t]
% \centering
% \resizebox{0.5\columnwidth}{!}{%
% \begin{tabular}{>{\centering\arraybackslash}m{2.3cm}|>{\centering\arraybackslash}m{1.2cm}>{\centering\arraybackslash}m{1.2cm}|>{\centering\arraybackslash}m{1.2cm}>{\centering\arraybackslash}m{1.2cm}}
% \hline
%  & \multicolumn{2}{c|}{AP 30 $\uparrow$} & \multicolumn{2}{c}{AP 50 $\uparrow$} \\ \hline
% (Hetero) Agents & 1 & 2 & 1 & 2 \\ \hline
% Late Fusion & 0.523  & 0.511 & 0.483 & 0.471 \\ 
% Calibrator & 0.520  & 0.524 & 0.484 & 0.488 \\ 
% E2E Training & 0.513  & 0.612 & 0.473 & 0.598 \\
% HEAL & 0.515  & 0.628 & 0.480 & \textbf{0.595} \\ 
% \cellcolor{pink!40} Ours & \cellcolor{pink!40} \textbf{0.523}  & \cellcolor{pink!40} \textbf{0.633} & \cellcolor{pink!40} \textbf{0.483} & \cellcolor{pink!40} 0.594 \\ \hline
% \end{tabular}%
% }
% \caption{Comparison of different methods under AP 30 and AP 50 metrics on the V2V4Real dataset}
% \label{tab:results_v2v4real}
% \end{table}

% \begin{figure*}[t]
% \centering
% \includegraphics[width=0.8\textwidth]{Figures/efficiency.pdf}
% \caption{}
% \label{fig:efficiency}
% \end{figure*}

\subsubsection{Efficiency Comparison}
\label{sec:eff}

We conducted an efficiency comparison between our approach and existing heterogeneous collaborative perception pipelines, focusing on the total number of parameters and training GPU hours. Training GPU hours refers to the time required to complete model training on the OPV2V dataset using an RTA A6000 GPU. To analyze training costs at scale, we report the number of training parameters and the estimated training time. \Figref{fig:efficiency} illustrates the changes in the number of training parameters and estimated training GPU hours as the number of heterogeneous agents increases from 1 to 12. End-to-end training and HEAL exhibit a steep increase in both parameters and GPU hours as the number of agents grows. In contrast, although our pipeline show higher parameters and GPU hours at the one or two number of agents (due to the training of the protocol model), it demonstrates a much slower growth rate because our proposed adapter $\upphi$ and reverter $\uppsi$ is very light-weighted and only takes 2 epochs to finish training. His highlights the scalability of our pipeline.

\help{Do I need to explain how the number of parameters and GPU hours are calculated? This is not a minor}
















% \subsection{Modal-agnostic Fusion}
\label{sec:modal_agnostic_fusion}




% \begin{table*}[t]
%     \centering
%     \resizebox{\textwidth}{!}{%
%     % \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
%     \begin{tabular}{ccccccccc}
%         \hline
%         \textbf{Model} & \textbf{Sensors} & \textbf{Backbone} & \textbf{Method} & \textbf{Range (m)} & \textbf{Resolution} & \textbf{Task} & \textbf{Fusion Method} \\
%         \hline
%         CoBevT (PMLR 2023)~\cite{xu2023cobevt}     & Camera/Lidar  & ResNet34+FAX          & PointPillar   & [-50,50,-50,50]               & 32$\times$32    & Seg      & Axial Attention \\ \hline
%         % HM-ViT (ICCV 2023)      & Camera+Lidar  & ResNet50+BevFormer    & PointPillar   & [-140,140,-40,40]               & 350$\times$100    & Det  & 3D Graph Attention \\ \hline
%         HEAL (ICLR 2024)~\cite{lu2024an}       & Camera/Lidar  & EfficientNet$^*$      & SECOND$^*$    & [-102.4, 102.4, -51.2, 51.2]    & 256$\times$128    & Det  & Pyramid Fusion \\ \hline
%     V2XVit (ECCV 2022)~\cite{xu2022v2x}         & Lidar         & -                     & PointPillar         & [-140.8, 140.8 -38.4, 38.4]               & 176$\times$48         & Det  & Window Attention \\ \hline
%         F-Cooper (ACM 2019)~\cite{chen2019f}     & Lidar         & -                     & VoxelNet      & [0, 70.4,-40,40]                & 352$\times$400    & Det  & max \\
%         \hline
%     \end{tabular}%
%     }
%     \caption{Comparison of Different Models}
%     \label{tab:models_comparison}
% \end{table*}


\subsection{Model and Task-agnostic Fusion}
\label{sec:task_agnostic_fusion}

% \begin{table*}[h]
%     \centering
% \resizebox{\textwidth}{!}{%
%     \begin{tabular}{c|c|cccc}
%         \Xhline{2\arrayrulewidth}
%         \multirow{8}{*}{\textbf{Agent Info}} & Hetero Agent Model & \textbf{Cobevt} & \textbf{Cobevt} & \textbf{HEAL} & \textbf{V2XViT} \\ 
%         \cline{2-6}
%         & Downstream Task & Static Seg & Dynamic Seg & Object Det & Object Det \\ 
%         % \cline{2-6}
%         & Sensor Modality & Lidar & Lidar & Camera & Lidar \\ 
%         % \cline{2-6}
%         & Backbone & PointPillar & PointPillar & EfficientNet-b0 & PointPillar \\ 
%         % \cline{2-6}
%         % & Visible Range (H, W) & \(100, 100\) & \(100, 100\) & \(102.4, 102.4\) & \(102.4, 76.8\) \\ 
%         % \cline{2-6}
%         & Feature Resolution & 32×32 & 32×32 & 128×128 & 64×48 \\ 
%         % \cline{2-6}
%         & Fusion Method & Axial Attention & Axial Attention & Pyramid Fusion & Window Attention \\ 
%         % \cline{2-6}
%         & Metric & MIoU & MIoU & AP 50 & AP 50 \\ 
%         \Xhline{2\arrayrulewidth}
%         \multirow{3}{*}{\shortstack{\textbf{Evaluation Result} \\ noise 0.0}} & Non-Collab & 0.507 & 0.641 & 0.347 & 0.861 \\ 
%         % \cline{2-6}
%         & w/o adpatation & 0.147 \textcolor{red}{($\minus$0.360)} & 0.066 \textcolor{red}{($\minus$0.575)} & 0.312 \textcolor{red}{($\minus$0.034)} & 0.898 \textcolor{blue}{(+0.037)} \\ 
%         % \cline{2-6}
%         & \cellcolor{pink!40} w/ adpatation (ours) & \cellcolor{pink!40} \textbf{0.561} \textcolor{blue}{(+0.054)} & \cellcolor{pink!40} \textbf{0.675} \textcolor{blue}{(+0.034)} & \cellcolor{pink!40} \textbf{0.677} \textcolor{blue}{(+0.365)} & \cellcolor{pink!40} \textbf{0.909} \textcolor{blue}{(+0.048)} \\ 
%         \Xhline{2\arrayrulewidth}
%         \multirow{3}{*}{\shortstack{\textbf{Evaluation Result} \\ noise 0.2}} & Non-Collab & 0.505 & 0.640 & 0.346 & 0.861 \\ 
%         % \cline{2-6}
%         & w/o adpatation & 0.136 \textcolor{red}{($\minus$0.370)} & 0.073 \textcolor{red}{($\minus$0.567)} & 0.313 \textcolor{red}{($\minus$0.036)} & 0.889 \textcolor{blue}{(+0.030)}\\ 
%         % \cline{2-6}
%         & \cellcolor{pink!40} w/ adpatation (ours) & \cellcolor{pink!40} \textbf{0.549} \textcolor{blue}{(+0.044)} & \cellcolor{pink!40} \textbf{0.669} \textcolor{blue}{(+0.029)} & \cellcolor{pink!40} \textbf{0.643} \textcolor{blue}{(+0.297)} & \cellcolor{pink!40} \textbf{0.904} \textcolor{blue}{(+0.043)} \\ 
%         \Xhline{2\arrayrulewidth}
%         \multirow{3}{*}{\shortstack{\textbf{Evaluation Result} \\ noise 0.4}} & Non-Collab & 0.503 & 0.630 & 0.339 & 0.859 \\ 
%         % \cline{2-6}
%         & w/o adpatation & 0.135 \textcolor{red}{($\minus$0.368)} & 0.072 \textcolor{red}{($\minus$0.567)} & 0.300 \textcolor{red}{($\minus$0.039)} & 0.874 \textcolor{blue}{(+0.015)} \\ 
%         % \cline{2-6}
%         & \cellcolor{pink!40} w/ adpatation (ours) & \cellcolor{pink!40} \textbf{0.523} \textcolor{blue}{(+0.020)} & \cellcolor{pink!40} \textbf{0.656} \textcolor{blue}{(+0.017)} & \cellcolor{pink!40} \textbf{0.513} \textcolor{blue}{(+0.213)} & \cellcolor{pink!40} \textbf{0.902} \textcolor{blue}{(+0.028)} \\ 
%         \Xhline{2\arrayrulewidth}
%     \end{tabular}%
% }
%     \caption{Heterogeneous collaborative perception results under the model and task-agnostic setting}
%     \label{tab:task_agnostic}
% \end{table*}


\begin{table*}[h]
    \centering
\resizebox{\textwidth}{!}{%
    \begin{tabular}{c|c|cccc}
        \Xhline{2\arrayrulewidth}
        \multirow{5}{*}{\textbf{Agent Info}} & Downstream Task & Object Det & Object Det & Static Seg & Dynamic Seg \\ 

        & Sensor Modality & Lidar & Camera & Lidar & Lidar \\ 
        % \cline{2-6}
        & Backbone & SECOND & EfficientNet-b0 & PointPillar & PointPillar \\ 
        & Fusion Method & Window Attention & Pyramid Fusion & Pyramid Fusion & Pyramid Fusion \\ 
        % \cline{2-6}
        & Metric & AP 50 & AP 50 & MIoU & MIoU \\ 
        \Xhline{2\arrayrulewidth}
        \multirow{3}{*}{\shortstack{\textbf{Evaluation} \\ ($\sigma: 0.0$)}} & Non-Collab & \textbf{0.908} & 0.399 & 0.548 & 0.675 \\ 
        % \cline{2-6}
        & w/o adpatation & 0.865 \textcolor{red}{($\minus$0.043)} & 0.399 (+0.000) & 0.114 \textcolor{red}{($\minus$0.434)} & 0.070 \textcolor{red}{($\minus$0.605)} \\ 
        % \cline{2-6}
        & \cellcolor{pink!40} w/ adpatation (ours) & \cellcolor{pink!40} 0.903 \textcolor{red}{($\minus$0.006)} & \cellcolor{pink!40} \textbf{0.760} \textcolor{blue}{(+0.362)} & \cellcolor{pink!40} \textbf{0.624} \textcolor{blue}{(+0.076)} & \cellcolor{pink!40} \textbf{0.690} \textcolor{blue}{(+0.014)} \\ 
        \Xhline{2\arrayrulewidth}
        \multirow{3}{*}{\shortstack{\textbf{Evaluation} \\ ($\sigma: 0.2$)}} & Non-Collab & \textbf{0.901} & 0.399 & 0.521 & 0.658 \\ 
        % \cline{2-6}
        & w/o adpatation & 0.859 \textcolor{red}{($\minus$0.041)} & 0.399 (+0.000) & 0.114 \textcolor{red}{($\minus$0.407)} & 0.069 \textcolor{red}{($\minus$0.588)}\\ 
        % \cline{2-6}
        & \cellcolor{pink!40} w/ adpatation (ours) & \cellcolor{pink!40} 0.892 \textcolor{red}{($\minus$0.009)} & \cellcolor{pink!40} \textbf{0.734} \textcolor{blue}{(+0.336)} & \cellcolor{pink!40} \textbf{0.615} \textcolor{blue}{(+0.094)} & \cellcolor{pink!40} \textbf{0.676} \textcolor{blue}{(+0.018)} \\ 
        \Xhline{2\arrayrulewidth}
        \multirow{3}{*}{\shortstack{\textbf{Evaluation} \\ ($\sigma: 0.4$)}} & Non-Collab & \textbf{0.881} & 0.399 & 0.503 & 0.630 \\ 
        % \cline{2-6}
        & w/o adpatation & 0.840 \textcolor{red}{($\minus$0.041)} & 0.400 \textcolor{blue}{(+0.001)} & 0.114 \textcolor{red}{($\minus$0.389)} & 0.069 \textcolor{red}{($\minus$0.561)} \\ 
        % \cline{2-6}
        & \cellcolor{pink!40} w/ adpatation (ours) & \cellcolor{pink!40} 0.861 \textcolor{red}{($\minus$0.020)} & \cellcolor{pink!40} \textbf{0.585} \textcolor{blue}{(+0.186)} & \cellcolor{pink!40} \textbf{0.600} \textcolor{blue}{(+0.097)} & \cellcolor{pink!40} \textbf{0.650} \textcolor{blue}{(+0.020)} \\ 
        \Xhline{2\arrayrulewidth}
    \end{tabular}%
}
    \caption{Heterogeneous collaborative perception results under the model and task-agnostic setting}
    \label{tab:task_agnostic}
\end{table*}


In this section, we evaluate the performance of our proposed pipeline in task-agnostic scenario on the OPV2V dataset. We choose four existing collaborative perception models with different input sensors and downstream tasks and equip then to each agent following the order based on the agent's index to simulate the heterogeneity between agents. \Tabref{tab:task_agnostic} shows some high-level information about these four models. Hetero agent 1 is equipped with Cobevt~\cite{xu2022cobevt} and lidar sensor to perform BEV static object segmentation, including lane lines and driving road. Hetero agent 2 is also equipped with Cobevt and lidar sensor but to perform BEV dynamic object segmentation which only includes vehicles on the road. Hetero agent 3 is equipped with HEAL~\cite{lu2024extensible} and camera sensor to perform 3D object detection task. Hetero agent 4 equipped with V2XVit~\cite{xu2022v2x} and lidar sensor to also perform 3D object detection task. For the static and dynamic segmentation task, model performance are evaluated on MIoU and for the 3D object detection task, model performance are evaluated on AP50 (Average Precision with IoU threshold 0.5).


In addition to our pipeline with collaborative adaptation, we conduct two experiments for comparison -- non-collaborative and collaborate without adaptation. Non-collaborative refers to single agent perception where no information sharing between agents. Collaborate without adaptation refers to performing intermediate fusion with other agents despite the domain gap. \Tabref{tab:task_agnostic} shows the evaluation results on the OPV2V dataset with artificially added Gaussian noise of standard deviation $0.0, 0.2, \text{and }0.4$. We can see that for the BEV segmentation task, collaboration with adaptation outperforms the single agent BEV segmentation, while collaboration without adaptation produces devastating performance drop comparing to single agent BEV segmentation. For the 3D object detection task, although collaboration without adaptation does not lead to dramatic performance drop, (for example, under noiseless scenario, only 0.034 drop on AP50 for agent 3),  but our pipeline result in huge performance boost. For example, our pipeline reaches 0.677 on AP 50 for agent 3 under the noiseless scenario, where single agent method only reaches 0.347, which is +0.365 boost on AP 50.




\subsection{Ablation Studies}
\label{sec:ablation}



% \begin{table}[h]
%     \centering
%     \begin{minipage}{.5\linewidth}
%         \centering
%         \begin{tabular}{c|c|c}
%         \hline
%         Loss Func & AP 30 $\uparrow$ & AP 50 $\uparrow$ \\ \hline 
%         $L_f$ + $L_d$ & 0.633 & 0.594 \\ \hline 
%         $L_f$ & 0.528 \textcolor{red}{($\minus$0.105)} & 0.482 \textcolor{red}{($\minus$0.112)} \\ \hline
%         $L_d$ & 0.529 \textcolor{red}{($\minus$0.104)} & 0.484 \textcolor{red}{($\minus$0.110)} \\ \hline
%         \end{tabular}
%         \label{tab:loss_func}
%         \caption{Ablation studies of each major component of the loss function for training local adapters and reverters.}
%     \end{minipage}%
%     \hspace{0.2cm}
%     \begin{minipage}{.45\linewidth}
%         \centering
%         \begin{tabular}{c|c|c|c}
%         \hline
%         Size & Param.(M) & AP 30 $\uparrow$ & AP 50 $\uparrow$ \\ \hline
%         L & 1.592 & 0.623 & 0.588 \\ \hline
%         M & 0.866 & \textbf{0.631} & \textbf{0.594} \\ \hline
%         S & 0.503 & \textbf{0.631} & 0.593 \\ \hline
%         T & 0.182 & \textbf{0.631} & 0.593 \\ \hline
%         \end{tabular}
%         \label{tab:protocol_size}
%         \caption{Ablation studies of different encoder sizes of the protocol models.}
%     \end{minipage}
% \end{table}



\begin{figure*}[t]
\includegraphics[width=\textwidth]{Figures/ablations.pdf}
\caption{ablations opv2v}
\label{figure:ablations}
\end{figure*}


\begin{figure*}[t]
\includegraphics[width=.7\textwidth]{Figures/ablations_v2v4real.pdf}
\caption{ablations v2v4real}
\label{figure:ablations_v2v4real}
\end{figure*}



In this section, we conduct ablation studies on two factors that may affect the performance of our pipeline: 1) The loss function for training adapter $\upphi$ and reverter $\uppsi$, and 2) the choice of protocol model's encoder size.

% \noindent \textbf{Loss Function}

% Our loss function consists $L_f$ to align BEV features in the intermediate feature space and $L_d$ to align BEV features in the decision space. As shown in \Tabref{tab:loss_func}, by removing $L_f$, the performance is dropped by 0.105 on AP 30 and 0.112 on AP 50. By removing $L_d$, the performance in dropped by 0.104 on AP 30 and 0.110 on AP 50. This shows that both $L_f$ and $L_d$ are important in our pipeline.

% \noindent \textbf{Protocol Encoder Size}

% In our pipeline, protocol model plays a cruel role in learning an unified BEV feature representation. It is reasonable to suspect that modifying the encoder size may affect the performance of collaborative adaptation. To this end, by changing the hidden size of protocol encoders. we experiment four different sizes of protocol encoders, L (Large), M (medium), S (small), and T (tiny), and keep the decoder invariant. Surprisingly, the experimental results in \Tabref{tab:protocol_size} shows that larger protocol encoder size does not necessarily lead to higher performance. Protocol model with medium, size, and tiny size result in very similar performance. \XG{Either find some arguable explanation, or do experiment on OPV2V dataset instead of V2V4Real dataset only}

% \noindent \textbf{BEV Feature Size}

% \XG{Experiments}

% \noindent \textbf{Different adapter and reverter archiectures}

% \XG{Experiments}

% \noindent \textbf{Protocol Model Task}

% \XG{Experiments}



==> sec/4_experiments_final_bk.tex <==
% \section{Experiments}

% One of the key contribution of our proposed MasCo framework is allowing agents with heterogeneous models and tasks to collaborate, requiring no sharing among local agents about model or task information. To our knowledge, our pipeline is the first one that achieves this goal. Therefore, to compare with other existing heterogeneous collaborative perception methods, in \Secref{sec:heter_agent}, we simplify the experiments to a single downstream task, 3D object detection, conducting comparison in object detection accuracy over the metric of average precision and training efficiency over trainable parameters and training GPU hours. Then, in \Secref{sec:task_agnostic_fusion}, we choose four existing collaborative models with heterogeneous model architectures and downstream tasks to evaluate the performance of our pipeline under the task-agnostic setting. Finally, we conduct ablation studies over the channel size, model architectures, and loss functions in \Secref{sec:ablation}.

% \subsection{Experimental Setups}
% \label{sec:implementation}
% \noindent \textbf{Dataset:} We conduct our experiment on two multi-agent collaborative perception datasets, a simulated dataset OPV2V\cite{xu2022opv2v}, and a real-world dataset V2V4Real\cite{xu2023v2v4real}. For multi-agent collaborative perception, simulated datasets are advantaged by their scale, such as the number of samples and the number of agents in each sample, as well as their diversified input modalities and downstream task annotations. For example, OPV2V contains 11k samples with 4 rgb images and 1 lidar point clouds inputs for each sample. Each sample contains 2-5 agents to performance collaborative perception. It also contains in total of 230k 3D bounding box annotations for the object detection task as well as both static and dynamic object segmentation annotations for the BEV segmentation task. On the other hand, real-world datasets are advantaged by their data realism which more accurately reflects the model performance in the real world. However, real-world datasets  such as V2V4Real only releases 20k samples with lidar point clouds inputs only. Each sample only contains 2 agents for collaborative perception. Besides, V2V4Real release 240K 3D bounding box annotations for 3D object detection task only. For a comprehensive experiments, in \Secref{sec:heter_agent}, we use both the simulated dataset OPV2V and the real-world dataset V2V4Real to compare our pipeline with existing heterogeneous collaborative perception pipeline under the object detection downsteam task. In \Secref{sec:task_agnostic_fusion}, since V2V4Real do not contain multiple tasks' annotations, we only use OPV2V to evaluate our pipeline under the task-agnostic setting. In \Secref{sec:ablation}, we use both datasets to conduct ablation studies.

\section{Experiments}
Our STAMP framework enables collaboration among agents with heterogeneous modalities, models architectures, and downstream tasks without sharing model or task information. We first compare our framework with existing heterogeneous CP frameworks in \Secref{sec:heter_agent}. Given that no previous work supports simultaneous task- and model-agnostic heterogeneous collaboration, we concentrate our evaluation on the 3D object detection task. This focus ensures a fair comparison across two key dimensions: object detection accuracy, measured by average precision, and training efficiency, assessed through trainable parameters and GPU hours required for training. Next, in \Secref{sec:task_agnostic_fusion}, we demonstrate our framework's unique capability in a task- and model-agnostic setting, evaluating its performance using four existing collaborative models with heterogeneous architectures and downstream tasks. Then, we present ablation studies on channel sizes, model architectures, and loss functions in \Secref{sec:ablation} to further analyze our framework's design choices. Finally, we present some feature and output visualization in \Secref{sec:vis}.

% \subsection{Experimental Setup}
% \label{sec:implementation}
% For our experiments, we utilize two multi-agent collaborative perception datasets: the simulated OPV2V \cite{xu2022opv2v} and the real-world V2V4Real \cite{xu2023v2v4real}. OPV2V contains 11k samples, each featuring 2-5 agents, with 4 RGB images and 1 LiDAR point cloud per sample. It provides annotations for both 3D object detection (230k bounding boxes) and BEV segmentation. V2V4Real, on the other hand, offers 20k samples with 2 agents each, providing only LiDAR point clouds and 240k 3D bounding box annotations for object detection.
% We employ both datasets in \Secref{sec:heter_agent} and \Secref{sec:ablation} to compare our pipeline with existing methods and conduct ablation studies. For the task-agnostic evaluation in \Secref{sec:task_agnostic_fusion}, we use only OPV2V due to its multi-task annotations. This combination of datasets allows us to leverage the advantages of both simulated and real-world data. The simulated dataset offers benefits in terms of scale, diversity of input modalities, and multi-task annotations, while the real-world dataset provides enhanced data realism, crucial for accurately assessing model performance in practical scenarios.



% \noindent \textbf{Implementation Details:} We have two different experimental setups for \Secref{sec:heter_agent} under 3D object detection setting and for \Secref{sec:task_agnostic_fusion} under the task agnostic setting. The detailed setups are illustrate within each section. For all experiments except end-to-end train strategy, local models and protocol models are trained for 30 epochs with Adam optimizer~\cite{kingma2014adam}. For end-to-end training, we increased the number of iterations proportionally to the number of agents, i.e., \(\text{Iters}_N = 30N\), where \(N\) represents the number of heterogeneous models. Local adapter $\upphi$ and local reverter $\uppsi$ are also trained with Adam optimizer but only for 5 epochs. We set the loss scaling factor $\lambda^f_\text{adapt} = \lambda^f_\text{revert} = \lambda^d_\text{adapt} = \lambda^d_\text{revert} = 0.5$. For more implementation details, please refer \Secref{sec:heter_agent}, \Secref{sec:task_agnostic_fusion}, and Appendix.


\subsection{Experimental Setup}
\label{sec:implementation}
Our experiments utilize two CP datasets: the simulated OPV2V dataset \citep{xu2022opv2v} and the real-world V2V4Real dataset \citep{xu2023v2v4real}. The OPV2V dataset provides $11k$ samples with each scene contains $2$ to $5$ agents, featuring RGB images and LiDAR point clouds, along with annotations for both 3D object detection (230k bounding boxes) and BEV segmentation. V2V4Real offers $20k$ samples with $2$ agents each, containing LiDAR point cloud inputs and 240k 3D bounding box annotations for object detection. We employ both datasets in \Secref{sec:heter_agent} and \Secref{sec:ablation} for method comparison and ablation studies. The task- and model-agnostic evaluation in \Secref{sec:task_agnostic_fusion} uses only OPV2V due to its multi-task annotations. This combination leverages the scale and diversity of simulated data with the realism of real-world data, ensuring comprehensive model evaluation.

\paragraph{Implementation details.}We use different setups for 3D object detection (\Secref{sec:heter_agent}) and task-agnostic settings (\Secref{sec:task_agnostic_fusion}), detailed within each section. Unless using end-to-end training, local and protocol models are trained for 30 epochs using Adam optimizer \citep{kingma2014adam}. For end-to-end training, we use $\text{Iters}_N = 30N$ epochs, where $N$ is the number of heterogeneous models, to ensure all models receive the same amount of supervision. Local adapters $\upphi$ and reverters $\uppsi$ are trained for 5 epochs. We set loss scaling factors $\lambda^f_\text{adapt} = \lambda^f_\text{revert} = \lambda^d_\text{adapt} = \lambda^d_\text{revert} = 0.5$ empirically. For additional details, please refer to \Secref{sec:heter_agent}, \Secref{sec:task_agnostic_fusion}, and Appendix \ref{X:model_appendix}.


\subsection{Heterogeneous Collaborative Perception For 3D Object Detection}
\label{sec:heter_agent}

\paragraph{Performance comparison.} We compare our method with existing heterogeneous CP approaches on the 3D object detection task. We select two late fusion methods (vanilla late fusion and calibrator \citep{xu2023model}) and two intermediate fusion methods (end-to-end training and HEAL \citep{lu2024extensible}) for comparison. Late fusion methods offer a simple way to mitigate domain gaps in collaborative 3D object detection. \cite{xu2023model} propose using a calibrator to address residual domain gaps in late fusion, which arise from differences in training data and procedures among heterogeneous models. For intermediate fusion, end-to-end training of all heterogeneous models together allows collaboration during the training stage to bridge domain gaps. \cite{lu2024extensible} introduce a backward alignment technique, first training a base network, then fixing its decoder while training only the encoders to create heterogeneous models. An architectural comparison between these frameworks and our proposed STAMP framework is illustrated and visualized in Appendix \ref{figure:cmp}.

We prepared 12 heterogeneous local models (six with LiDAR modality and six with RGB camera modality) and one protocol model with LiDAR modality (details in Appendix \ref{X:model_appendix}). Each agent has a visible range of $51.2\text{m} \times 51.2\text{m}$ square units. Considering that most samples of the OPV2V dataset contain no more than four agents, we only select the first four models for evaluation on the OPV2V dataset. Similarly, we select the first two models for the V2V4Real dataset since it has two agents for each sample. All 12 models are used for efficiency comparison.


\begin{table*}[t]
\caption{Performance comparison using AP@30 and AP@50 metrics on the OPV2V dataset. Agent positions are perturbed with Gaussian noise of standard deviations 0.0, 0.2, and 0.4.}
% \vspace{\baselineskip}
\vspace{1mm}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{>{\centering\arraybackslash}m{0.8cm}|>{\centering\arraybackslash}m{2.3cm}|>{\centering\arraybackslash}m{1.2cm}>{\centering\arraybackslash}m{1.2cm}>{\centering\arraybackslash}m{1.2cm}>{\centering\arraybackslash}m{1.2cm}|>{\centering\arraybackslash}m{1.2cm}>{\centering\arraybackslash}m{1.2cm}>{\centering\arraybackslash}m{1.2cm}>{\centering\arraybackslash}m{1.2cm}}
\toprule
& & \multicolumn{4}{c|}{\textbf{AP@30} $\uparrow$} & \multicolumn{4}{c}{\textbf{AP@50} $\uparrow$} \\ 
% \Xhline{2\arrayrulewidth}
\midrule
$\sigma$ & Agent Index & \textbf{Agent 1} & \textbf{Agent 2} & \textbf{Agent 3} & \textbf{Agent 4} & \textbf{Agent 1} & \textbf{Agent 2} & \textbf{Agent 3} & \textbf{Agent 4} \\ 
% \Xhline{2\arrayrulewidth}
\midrule

\multirow{5}{*}{0.0}    & Late Fusion     & \textbf{0.902}    & 0.931             & 0.935             & 0.935             & 0.894             & 0.908             & 0.913             & 0.914 \\
                        & Calibrator      & 0.901             & 0.935             & 0.939             & 0.938             & \textbf{0.896}    & 0.914             & 0.916             & 0.920 \\
                        & E2E Training    & 0.899             & 0.973             & 0.978             & 0.986             & 0.885             & 0.967             & 0.977             & 0.980 \\
                        & HEAL            & 0.897             & 0.975             & 0.986             & 0.985             & 0.889             & 0.972             & 0.978             & 0.983 \\
                        & \cellcolor{pink!40} STAMP (ours)            & \cellcolor{pink!40} \textbf{0.902}    & \cellcolor{pink!40} \textbf{0.981}    & \cellcolor{pink!40} \textbf{0.987}    & \cellcolor{pink!40} \textbf{0.989}    & \cellcolor{pink!40} 0.894             & \cellcolor{pink!40} \textbf{0.977}    & \cellcolor{pink!40} \textbf{0.983}    & \cellcolor{pink!40} \textbf{0.985} \\ 
                        % \Xhline{2\arrayrulewidth}
                        \midrule

\multirow{5}{*}{0.2}    & Late Fusion     & \textbf{0.900}    & 0.910             & 0.902             & 0.905             & 0.882             & 0.783             & 0.797             & 0.792 \\
                        & Calibrator      & 0.897             & 0.908             & 0.898             & 0.902             & \textbf{0.885}    & 0.778             & 0.800             & 0.791 \\
                        & E2E Training    & \textbf{0.900}    & 0.967             & 0.961             & 0.961             & 0.879             & 0.936             & 0.941             & 0.934 \\
                        & HEAL            & 0.899             & 0.971             & 0.965             & 0.962             & 0.881             & \textbf{0.938}    & 0.940             & 0.940 \\
                        & \cellcolor{pink!40} STAMP (ours)            & \cellcolor{pink!40} \textbf{0.900}    &  \cellcolor{pink!40} \textbf{0.975}    & \cellcolor{pink!40} \textbf{0.968}    & \cellcolor{pink!40} \textbf{0.968}    & \cellcolor{pink!40} 0.882             & \cellcolor{pink!40} 0.937              & \cellcolor{pink!40} \textbf{0.948}    & \cellcolor{pink!40} \textbf{0.946} \\ 
                        % \Xhline{2\arrayrulewidth}
                        \midrule





\multirow{5}{*}{0.4}    & Late Fusion     & \textbf{0.888}    & 0.882             & 0.864             & 0.870             & \textbf{0.874}    & 0.639             & 0.614             & 0.617 \\ 
                        & Calibrator      & 0.874             & 0.889             & 0.887             & 0.871             & 0.867             & 0.644             & 0.622             & 0.628 \\ 
                        & E2E Training    & 0.885             & 0.952             & 0.956             & 0.952             & 0.863             & 0.883             & 0.892             & 0.899 \\ 
                        & HEAL            & 0.880             & 0.959             & 0.961             & 0.962             & 0.852             & 0.913             & \textbf{0.915}    & \textbf{0.912} \\ 
                        & \cellcolor{pink!40} STAMP (ours)            & \cellcolor{pink!40} \textbf{0.888}    & \cellcolor{pink!40} \textbf{0.961}    & \cellcolor{pink!40} \textbf{0.963}    & \cellcolor{pink!40} \textbf{0.966}    & \cellcolor{pink!40} \textbf{0.874}    & \cellcolor{pink!40} \textbf{0.915}    & \cellcolor{pink!40} \textbf{0.915}    & \cellcolor{pink!40} 0.909 \\ \bottomrule
\end{tabular}%
}
\vspace{-5mm}
\label{tab:results_opv2v}
\end{table*}

For the OPV2V dataset, we simulate real-world noise by adding Gaussian noise with standard deviations $\sigma = \{0.0, 0.2, 0.4\}$ to the agents' locations. As shown in Table \ref{tab:results_opv2v}, late fusion methods underperform as the number of agents increases, with performance degrading further at higher noise levels $(\sigma = 0.4)$. This is particularly evident when camera agents (agents 3 and 4) are involved, highlighting the late fusion methods' vulnerability to bottleneck agents' incorrect predictions. Our framework demonstrates superior or comparable performance to other heterogeneous fusion methods across all noise levels. 


\begin{wraptable}{r}{0.52\textwidth}
\vspace{-7mm}
\caption{Performance comparison using AP@30 and AP@50 metrics on the V2V4Real dataset.}
% \vspace{\baselineskip}
\vspace{1mm}
\centering
\resizebox{0.5\textwidth}{!}{
\begin{tabular}{>{\centering\arraybackslash}m{2.1cm}|>{\centering\arraybackslash}m{1.3cm}>{\centering\arraybackslash}m{1.3cm}|>{\centering\arraybackslash}m{1.3cm}>{\centering\arraybackslash}m{1.3cm}}
\toprule
 & \multicolumn{2}{c|}{\textbf{AP@30} $\uparrow$} & \multicolumn{2}{c}{\textbf{AP@50} $\uparrow$} \\ 
 % \Xhline{2\arrayrulewidth}
 \midrule
Agent Index & \textbf{Agent 1} & \textbf{Agent 2} & \textbf{Agent 1} & \textbf{Agent 2} \\ 
% \Xhline{2\arrayrulewidth}
\midrule
Late Fusion & 0.523  & 0.511 & 0.483 & 0.471 \\ 
Calibrator & 0.520  & 0.524 & 0.484 & 0.488 \\ 
E2E Training & 0.513  & 0.612 & 0.473 & 0.598 \\
HEAL & 0.515  & 0.628 & 0.480 & \textbf{0.595} \\ 
\cellcolor{pink!40} STAMP (ours) & \cellcolor{pink!40} \textbf{0.523}  & \cellcolor{pink!40} \textbf{0.633} & \cellcolor{pink!40} \textbf{0.483} & \cellcolor{pink!40} 0.594 \\ \bottomrule
\end{tabular}}
\label{tab:results_v2v4real}
\vspace{-3mm}
\end{wraptable}

\Tabref{tab:results_v2v4real} compares the average precision on the real-world V2V4Real dataset. Our STAMP pipeline demonstrates superior performance, achieving the highest AP@30 for both agents (0.523 and 0.633) and competitive AP@50 scores. STAMP outperforms Late Fusion methods and matches or exceeds the performance of existing heterogeneous intermediate fusion approaches like HEAL. These results indicate that the CFA module in STAMP is effective not only in simulated environments but also in real-world scenarios.


\begin{wrapfigure}{r}{0.52\textwidth}
\vspace{-2mm}
\centering
\includegraphics[width=0.5\textwidth]{Figures/efficiency.pdf}
\vspace{-3mm}
\caption{Training efficiency comparison of our framework and existing heterogeneous CP frameworks across a number of heterogeneous agents.}
\label{fig:efficiency}
\vspace{-3mm}
\end{wrapfigure}

\paragraph{Efficiency comparison.}We conducted an efficiency comparison between our approach and existing heterogeneous CP pipelines, focusing on the total number of parameters and training GPU hours. Training GPU hours refers to the time required to complete model training on the OPV2V dataset using an RTA A6000 GPU. To analyze training costs at scale, we report the number of training parameters and the estimated training time. \Figref{fig:efficiency} illustrates the changes in the number of training parameters and estimated training GPU hours as the number of heterogeneous agents increases from 1 to 12. End-to-end training and HEAL exhibit a steep increase in both parameters and GPU hours as the number of agents grows. In contrast, although our pipeline shows higher parameters and GPU hours at the one or two number of agents (due to the training of the protocol model), it demonstrates a much slower growth rate because our proposed adapter $\upphi$ and reverter $\uppsi$ is very light-weighted and only takes 5 epochs to finish training. This highlights the scalability of our pipeline.

\label{sec:modal_agnostic_fusion}


\subsection{Model- and Task-agnostic Fusion}
\label{sec:task_agnostic_fusion}

In this section, we evaluate our proposed framework's performance in a task-agnostic setting using the OPV2V dataset. To simulate agent heterogeneity, we assign four agents with diverse input sensors, learning objectives, and evaluation metrics, equipping them with various backbones and fusion models. 
%
Agent 1 was equipped with a SECOND encoder \citep{yan2018second} and a window attention fusion module \citep{xu2022v2x}. For Agent 2, we implemented an EfficientNet-b0 encoder \citep{tan2019efficientnet}, while Agents 3 and 4 were equipped with PointPillar encoders \citep{lang2019pointpillars}. Agents 2, 3, and 4 all utilized the Pyramid Fusion module \cite{lu2024extensible}.
%
Table \ref{tab:task_agnostic} summarizes these models' key characteristics. We compare our STAMP framework against two baseline scenarios: non-collaborative (single-agent perception without information sharing) and collaborative without feature alignment (performing intermediate fusion despite domain gaps). Table \ref{tab:task_agnostic} presents the evaluation results on the OPV2V dataset, with added Gaussian noise (standard deviations $\sigma=\{0.0, 0.2, 0.4\}$) to the agents' locations.

\begin{table*}[h]
\caption{Heterogeneous CP results in a model- and task-agnostic setting. Tasks include 3D object detection (`Object Det'), static object BEV segmentation (`Static Seg'), and dynamic object BEV segmentation (`Dynamic Seg'). 3D object detection is evaluated using Average Precision at 50\% IoU threshold (AP@50), while segmentation tasks use Mean Intersection over Union (MIoU).}
\vspace{2mm}

\centering
\resizebox{\textwidth}{!}{%
    \begin{tabular}{>{\centering\arraybackslash}m{2cm}|>{\centering\arraybackslash}m{2.8cm}|>{\centering\arraybackslash}m{2.6cm}>{\centering\arraybackslash}m{2.6cm}>{\centering\arraybackslash}m{2.6cm}>{\centering\arraybackslash}m{2.6cm}}
        % \Xhline{2\arrayrulewidth}
        \toprule
        \multirow{8}{*}{\textbf{Agent Info}} & Agent Index & \textbf{Agent 1} & \textbf{Agent 2} & \textbf{Agent 3} & \textbf{Agent 4} \\ 
        \cmidrule[0.5pt]{2-6}
        & Metric & AP@50 & AP@50 & MIoU & MIoU \\ 
        % \cline{2-6}
        % \cmidrule[0.5pt]{2-6}
        & Downstream Task & Object Det & Object Det & Static Seg & Dynamic Seg \\ 
        & Sensor Modality & Lidar & Camera & Lidar & Lidar \\ 
        % \cline{2-6}
        & Backbone & SECOND & EfficientNet-b0 & PointPillar & PointPillar \\ 
        & Feature Resolution & $64\times64$ & $128\times128$ & $128\times128$ & $128\times128$ \\ 
        & Channel Size & $256$ & $64$ & $64$ & $64$ \\ 
        & Fusion Method & Window Attention & Pyramid Fusion & Pyramid Fusion & Pyramid Fusion \\ 
        % \cline{2-6}
        % & Metric & \textbf{AP@50} & \textbf{AP@50} & \textbf{MIoU} & \textbf{MIoU} \\ 
        % \Xhline{2\arrayrulewidth}
        \midrule
        \multirow{3}{*}{\shortstack{\textbf{Evaluation} \\ ($\sigma: 0.0$)}} & Non-Collab & \textbf{0.941} & 0.399 & 0.548 & 0.675 \\ 
        % \cline{2-6}
        & Collab w/o. CFA & 0.909 \textcolor{red}{($\minus$0.032)} & 0.399 (+0.000) & 0.114 \textcolor{red}{($\minus$0.434)} & 0.070 \textcolor{red}{($\minus$0.605)} \\ 
        % \cline{2-6}
        & \cellcolor{pink!40} STAMP (ours)  & \cellcolor{pink!40} 0.936 \textcolor{red}{($\minus$0.005)} & \cellcolor{pink!40} \textbf{0.760} \textcolor{blue}{(+0.362)} & \cellcolor{pink!40} \textbf{0.624} \textcolor{blue}{(+0.076)} & \cellcolor{pink!40} \textbf{0.690} \textcolor{blue}{(+0.014)} \\ 
        % \Xhline{2\arrayrulewidth}
        \midrule
        \multirow{3}{*}{\shortstack{\textbf{Evaluation} \\ ($\sigma: 0.2$)}} & Non-Collab & \textbf{0.936} & 0.399 & 0.521 & 0.658 \\ 
        % \cline{2-6}
        & Collab w/o. CFA & 0.902 \textcolor{red}{($\minus$0.034)} & 0.399 (+0.000) & 0.114 \textcolor{red}{($\minus$0.407)} & 0.069 \textcolor{red}{($\minus$0.588)}\\ 
        % \cline{2-6}
        & \cellcolor{pink!40} STAMP (ours) & \cellcolor{pink!40} 0.930 \textcolor{red}{($\minus$0.006)} & \cellcolor{pink!40} \textbf{0.734} \textcolor{blue}{(+0.336)} & \cellcolor{pink!40} \textbf{0.615} \textcolor{blue}{(+0.094)} & \cellcolor{pink!40} \textbf{0.676} \textcolor{blue}{(+0.018)} \\ 
        % \Xhline{2\arrayrulewidth}
        \midrule
        \multirow{3}{*}{\shortstack{\textbf{Evaluation} \\ ($\sigma: 0.4$)}} & Non-Collab & \textbf{0.925} & 0.399 & 0.503 & 0.630 \\ 
        % \cline{2-6}
        & Collab w/o. CFA & 0.886 \textcolor{red}{($\minus$0.039)} & 0.400 \textcolor{blue}{(+0.001)} & 0.114 \textcolor{red}{($\minus$0.389)} & 0.069 \textcolor{red}{($\minus$0.561)} \\ 
        % \cline{2-6}
        & \cellcolor{pink!40} STAMP (ours) & \cellcolor{pink!40} 0.923 \textcolor{red}{($\minus$0.002)} & \cellcolor{pink!40} \textbf{0.585} \textcolor{blue}{(+0.186)} & \cellcolor{pink!40} \textbf{0.600} \textcolor{blue}{(+0.097)} & \cellcolor{pink!40} \textbf{0.650} \textcolor{blue}{(+0.020)} \\ 
        % \Xhline{2\arrayrulewidth}
        \bottomrule
    \end{tabular}%
\vspace{\baselineskip}
}
\label{tab:task_agnostic}
\end{table*}

Our method consistently outperforms single-agent segmentation for agents 3 and 4 in the BEV segmentation task. Conversely, collaboration without feature alignment significantly degrades performance compared to the single-agent baseline, underscoring the importance of our adaptation mechanism in aligning heterogeneous features. For agent 2's camera-based 3D object detection, our pipeline achieves substantial gains (e.g., AP@50 improves from 0.399 to 0.760 in noiseless conditions), while collaboration without feature alignment shows negligible changes. These results demonstrate our pipeline's effectiveness in bridging domain gaps between heterogeneous agents, enabling successful collaboration across diverse models, sensors, and tasks. The consistent improvements, particularly under noisy conditions, highlight our approach's robustness and adaptability.

However, we observe that both collaborative approaches lead to performance degradation for Agent 1 compared to its single-agent baseline, despite our method outperforming collaboration without feature alignment. This unexpected outcome is attributed to Agent 2's limitations, which rely solely on less accurate camera sensors for 3D object detection. This scenario illustrates a bottleneck effect, where a weaker agent constrains the overall system performance, negatively impacting even the strongest agents. This challenge in multi-agent collaboration systems prompts us to introduce the concept of a \textbf{Multi-group Collaboration System}. In Appendix~\ref{X:discussion}, we elaborate on the advantages of such a system and demonstrate how our framework can be easily integrated to potentially mitigate performance discrepancies in heterogeneous agent collaborations.


\subsection{Ablation Studies}
\label{sec:ablation}





In this section, we conduct ablation studies on three factors that may affect our pipeline's performance: BEV feature channel size, adapter \& reverter architectures, and loss functions for collaborative feature alignment. All experiments are conducted on both the OPV2V and V2V4Real datasets.


\begin{figure*}[ht]
\includegraphics[width=\textwidth]{Figures/ablation_opv2v.pdf}
\vspace{-5mm}
\caption{Ablation studies on the OPV2V dataset: (a) Model performance across different BEV feature channel sizes. (b) Performance comparison of various adapter and reverter architectures. (c) Performance results using different combinations of loss function components ($L_f$ and $L_d$).}
\label{figure:ablations}
\end{figure*}



\begin{wrapfigure}{r}{0.5\textwidth}
\vspace{-3mm}
\includegraphics[width=.5\textwidth]{Figures/ablations_v2v4real.pdf}
\vspace{-5mm}
\caption{Ablation studies on the V2V4real set.}
\label{figure:ablations_v2v4real}
\vspace{-3mm}
\end{wrapfigure}

\paragraph{BEV feature channel size.}Changing the BEV feature channel size is essentially a form of feature compression, which is crucial for controlling communication bandwidth in multi-agent collaboration systems. Our collaborative feature alignment module inherently supports feature compression by adjusting the protocol BEV feature's channel size. We experiment with two channel sizes for the protocol BEV feature, 32 and 16, and compare their performance to our standard implementation with a channel size of 64 (Figures \ref{figure:ablations} and \ref{figure:ablations_v2v4real}). Surprisingly, reducing the channel size results in only minor performance changes for both datasets, revealing our model's resilience to high BEV feature compression rates.

\paragraph{Adapter \& reverter architecture.}We evaluate two alternative architectures for the adapter and reverter—a single $1\times1$ convolutional layer and three self-attention layers—compared to our standard implementation of three ConvNeXt layers. The results demonstrate that performance is not highly sensitive to the adapter and reverter architecture, showcasing our framework's flexibility across various specific implementations.

\paragraph{Loss function.}The final loss function in our collaborative feature alignment module comprises two components: $L_f$ for feature space alignment and $L_d$ for decision space alignment. We evaluate our method's performance using each loss function individually. Figure \ref{figure:ablations} shows that on the OPV2V dataset, using only $L_d$ leads to a significant performance drop, while using only $L_f$ results in more fluctuating and generally lower performance. Figure \ref{figure:ablations_v2v4real} demonstrates that on the V2V4Real dataset, dropping either $L_d$ or $L_f$ results in performance degradation. These findings underscore the necessity of using both loss functions in combination for optimal performance.

==> sec/intro_revising_version.tex <==
\section{Introduction}
\label{sec:intro}
Multi-agent collaborative perception \citep{bai2022survey, han2023collaborative, liu2023towards} has emerged as a promising solution for autonomous systems, leveraging communications from multiple connected agents. It enables agents (e.g., vehicles, infrastructure) to share perceptual information, providing a more comprehensive view of the environment. Despite its potential, collaborative perception faces significant challenges, particularly when dealing with heterogeneous agents with different input modalities, model parameters, architectures, or learning objectives. \cite{xu2023bridging} observed that features of heterogeneous agents are dissimilar in spatial resolution, channel number, and feature patterns. This domain gap hinders effective and efficient collaborative perception when employing fusion-based approaches. 

To enable collaboration among heterogeneous agents, $i.e.$ heterogeneous collaboration, one might consider using early or late fusion instead of intermediate fusion. However, early fusion requires high communication bandwidth while late fusion often results in suboptimal accuracy and it is not viable across models with different downstream tasks. Alternative approaches attempt to achieve heterogeneous intermediate fusion by either adding pair-wise adapters \citep{xu2023bridging} or sharing part of the models \citep{lu2024extensible}. While effective in bridging the domain gap, these methods are limited in scalability or security, rendering them insufficiently practical for real-world applications. Recent studies have also highlighted increased security vulnerabilities in collaborative perception systems compared to single-agent systems \citep{hu2024collaborative, tu2021adversarial, li2023among}. Notably, \cite{li2023among} found that black-box attacks are nearly ineffective without the knowledge of other agents' models, emphasizing the importance of task and model-agnostic approaches in enhancing system security against adversarial threats.

To address these challenges, we propose \textbf{STAMP}, a scalable task and model-agnostic collaborative perception framework. Our approach employs lightweight adapter and reverter pairs to transform the Bird's Eye View (BEV) features of each heterogeneous agent into a unified protocol BEV feature domain. These protocol BEV features are then broadcasted to other agents and subsequently mapped back to their corresponding local domains, enabling collaboration within each agent's local domain. We refer to this process as \textbf{Collaborative Feature Alignment (CFA)}. Our proposed pipeline offers several key advantages. Firstly, it enables existing heterogeneous agents to collaborate with minimal additional disk memory ($\sim$1MB) and computational overhead, making it scalable for a large number of heterogeneous agents. Secondly, the alignment process is designed to be task and model-agnostic, allowing our framework to integrate with various models and tasks without retraining the model or the need to share models among agents. This enhances both the flexibility and security of the system.

We conducted comprehensive experiments to evaluate our collaborative perception pipeline's performance. Using the simulated OPV2V dataset \citep{xu2022opv2v} and the real-world V2V4Real dataset \citep{xu2023v2v4real}, we demonstrated that our pipeline achieves comparable or superior accuracy with a significantly lower training resource growth rate as the number of heterogeneous agents increases. Our method requires, on average, only 2.36 GPU hours of training time per additional agent, compared to 17.07 GPU hours per additional agent for existing heterogeneous collaborative pipelines. We also demonstrated our pipeline's unique ability to perform task- and model-agnostic collaboration, a capability not supported in existing methods. This achievement establishes a new benchmark for heterogeneous collaborative perception in autonomous driving, showcasing clear performance improvements in scenarios where other methods are unable to operate.

% \XG{Question: Do we really need the this bullet points (summary)? Or may need to be revised}

% The main contributions of this work can be summarized as follows:
% \begin{itemize}[leftmargin=10pt]
% \item We propose STAMP, a scalable task- and model-agnostic collaborative perception pipeline that enables effective collaboration among heterogeneous agents with minimal additional resources. It is open-sourced and supports multiple existing collaborative perception methods.
% \item We introduce Collaborative Feature Alignment (CFA). It allows heterogeneous agents to collaborate by sharing information in a unified protocol domain and keep the local feature map secure.
% \item We demonstrate comparable or superior accuracy with significantly lower training resource usage on the 3D object detection task, while showcasing our unique ability for task- and model-agnostic collaboration with clear performance improvements.
% \end{itemize}

% \ZT{Here missing a summary of contributions.}
